Test Coverage for Network Configurations

We develop NetCov, the first tool to reveal which network configuration lines are being tested by a suite of network tests. It helps network engineers improve test suites and thus increase network reliability. A key challenge in its development is that many network tests test the data plane instead of testing the configurations (control plane) directly. We must be able to efficiently infer which configuration elements contribute to tested data plane elements, even when such contributions are non-local (on remote devices) or non-deterministic. NetCov uses an information flow graph based model that precisely captures various forms of contributions and a scalable method to lazily infer contributions. Using it, we show that an existing test suite for Internet2 (a nation-wide backbone network in the USA) covers only 26% of the configuration lines. The feedback from NetCov makes it easy to define new tests that improve coverage. For Internet2, adding just three such tests covers an additional 17% of the lines.

==> Control-Plane-Coverage [arxiv submission] (4)/sections/abstract.tex <==
%\begin{abstract}
\textbf{Abstract---}
We develop \sysname, the first tool to reveal which network configuration lines are being tested by a suite of network tests. It helps network engineers improve test suites and thus increase network reliability.  A key challenge in its development is that many network tests test the data plane instead of testing the configurations (control plane) directly. We must be able to efficiently infer which configuration elements contribute to tested data plane elements, even when such contributions are non-local (on remote devices) or non-deterministic.
%
\sysname uses an information flow graph based model that precisely captures various forms of contributions and a scalable method to lazily infer contributions.
%
Using it, we show that an existing test suite for Internet2 (a nation-wide backbone network in the USA) covers only 26\% of the configuration lines. The feedback from \sysname makes it easy to define new tests that improve coverage. For Internet2, adding just three such tests covers an additional 17\% of the lines. 


% In the battle towards reliable networks, earlier research has pushed the limits of \textit{what can be tested} but leaves the question of \textit{what need to be tested}.
% As a result, even the best sort of verification tools today is being poorly applied.
% %Recent research on data plane coverage metrics proposed to quantify test completeness using the proportion of exercised data plane elements, such as forwarding rules. 


% To address this gap, we present \textit{configuration coverage} to measure test completeness and answer \textit{what are not tested}. Compared to data plane coverage metrics proposed by recent study, it considers all configuration elements instead of only the ones that contribute to the current data plane. It also directly locates testing gaps to specific lines. Defining and computing configuration coverage is challenging because some network tests exercise the data plane, \IE, the output of configurations, so we need to map the output back to configurations that contribute to it. %Such contributions are complex, \EG, any data plane element can be resulted from configuration elements across multiple routers. 
% We introduce a graph-based model that supports various forms of contributions--direct or indirect, strong or weak. We also propose a novel algorithm to infer the contributions on demand, and thus avoid the cost to track them proactively during data plane generation.

% We build a system called \sysname and it is open source. Our case study on Internet2 shows that existing tests have low coverage of 36\%. We also show that coverage can be effectively improved using the feedback provided by \sysname.
%\end{abstract}

==> Control-Plane-Coverage [arxiv submission] (4)/sections/background.tex <==
\section{Background on Network Testing} 
\label{sec:background}

In networks with distributed control planes, each device runs one or more routing protocol (e.g., BGP, OSPF) instances. Each instance exchanges routing messages with its neighboring instances. Routing messages contain attributes of paths that the sender is using to various destinations. A routing instance may learn multiple paths to the same destination via different neighbors. It selects the best one (or multiple best ones if multipath routing is enabled) based on its policy and stores that path in its protocol RIB (routing information base). 
%Each routing instances 
%deal with different path attributes and 
% maintain separate protocol RIBs. 
Multiple routing protocol instances on a device may have best paths to the same destination. The device selects the best one(s) based on the relative preference of the protocols and stores the selection in its main RIB. 
Information in the main RIB is used to forward packets.\footnote{In reality, for fast forwarding, routers have a forwarding information base (FIB), which maps each main RIB destination to its outgoing interface, by recursively resolving next hop information (which may be an IP address). The difference between main RIB and FIB is not material for our work, and we use the term main RIB for the table that has forwarding information.}

Network engineers can control many aspects of the computation above using device configuration. This includes the routing protocol instances that are running; the peering between instances; the destination prefixes that are announced by each routing protocol instance; how routing messages are transformed prior to sending (export policy) and upon reception (import policy); and the preference function for best path selection. Naturally, thus, how the network forwards packets is intimately dependent on device configurations.

Given the importance of configurations to correct network behavior, network engineers use automatic testing and verification to find bugs and gain confidence in their correctness. Network tests come in two flavors. {\em Data plane tests} analyze the computed data plane state (\IE, RIBs), e.g.,
%\footnote{While RIBs are routing tables---and routing is a control plane function---RIB entries are data plane state generated by running the control plane.} 
checking that node A can reach B and that route to a particular destination is present at node C. {\em Control plane tests} directly analyze device configuration, e.g., checking  that the import policy blocks routing messages for private address space (such as 10.0.0.0/8) and BGP peerings are correctly configured. 


% \section{Why Configuration Coverage} 
% \label{sec:background}

% \para{Background on network testing} 
% In networks with distributed control planes, each device runs one or more routing protocol (e.g., BGP, OSPF) instances. Each instance exchanges routing messages with its neighboring instances. Routing messages contain attributes of paths that the sender is using to various destinations. A routing instance may learn multiple paths to the same destination via different neighbors. It selects the best one (or multiple best ones if multipath routing is enabled) based on its policy and stores that in its protocol RIB (routing information base). 
% %Each routing instances 
% %deal with different path attributes and 
% % maintain separate protocol RIBs. 
% Multiple routing protocol instances on a device may have best paths to the same destination. The device selects the best one(s) based on the relative preference of the protocols and stores the selection in its main RIB. 
% Information in the main RIB is used to forward packets.\footnote{In reality, for fast forwarding, routers have a forwarding information base (FIB), which maps each main RIB destination to its outgoing interface, by recursively resolving next hop information (which may be an IP address). The difference between main RIB and FIB is not material for our work, and we use the term main RIB for the table that has forwarding information.}

% Network engineers can control all aspect of the computation above using device configuration. This includes which routing protocol instances are running; which instances peer with each other; which destination prefixes are announced by each routing protocol instance; how routing messages are transformed prior to sending (export policy) and upon reception (import policy); and the preference function for best path selection. Naturally, thus, how the network forwards packets is intimately dependent on device configurations.

% Given the importance of configurations to correct network behavior, network engineers use automatic testing and verification to find bugs and gain confidence in their correctness. Network tests come in two flavors. {\em Data plane tests} analyze the computed data plane state (\IE, RIBs), e.g.,
% %\footnote{While RIBs are routing tables---and routing is a control plane function---RIB entries are data plane state generated by running the control plane.} 
% checking that node A can reach B and that route to a particular destination is present at node C. {\em Control plane tests} directly analyze device configuration, e.g., checking  that the import policy blocks routing messages for private address space (such as 10.0.0.0/8) and BGP peerings are correctly configured. 

% %In testing terminology~\cite{xx}, one can think of data plane tests as integration tests and control plane tests as unit tests. The two types of tests have complementary properties. Unit tests enable rigorous testing of individual components, but they do not provide any assurance of end-to-end behaviors. Integration tests enable testing  end-to-end behaviors, but they may not rigorously test individual components.

% \para{A motivating example}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/motivation_example.png}
%     \vspace{-20pt}
%     \caption{An example data center network and parts of B2's configuration.}
%     \label{fig:example}
% \end{figure}

% Finding and minimizing gaps in configuration testing is important. If key elements of configuration are untested, networks with even the most sophisticated testing are vulnerable to outages. Consider the data center network in Figure \ref{fig:example}. It has eight leaf routers (L1$\cdots$L8), four spine routers (S1$\cdots$S4), and two border routers (B1, B2) that connect to a wide-area network (WAN). All routers run BGP and peer with each of their neighbors. The WAN routers, which are not administered by the data center engineers, announce paths to external destinations.

% Parts of B2's configuration is on the right (in pseudocode, not a real router vendor's language). Lines 2-3 define B2's peering with the WAN router and specify the import policy to use. This policy, defined on Lines 7-12, specifies what do with routing messages for prefixes in the prefix list \code{INTERNAL} and for the others. The prefix list includes all internal prefixes (Line 15).  We elide elements of B2's configuration related to interfaces and other BGP peers.

% Suppose the network uses three tests: $1)$ check that all leafs can reach each other; $2)$ check that  all leafs can reach the outside world by ensuring reachability to a few sentinel destinations (e.g., Google DNS); and $3)$ check that all leaf-spine, spine-border, and border-WAN BGP peerings are configured. 

% This test suite is comprehensively testing internal and external application flow paths and routing adjacencies. It also covers many elements of B2's configuration. The BGP peering configuration is covered by the third test; and parts of the \code{from-wan} import policy are covered by second test because reachability to external destinations depends on the import policy permitting those destinations.

% %Further, it is exercising not only the configurations of leaf routers (where flows start) but also of spine and border routers that make the WAN reachable by leaf routers. For instance, if BGP peering between the border routers and the WAN were misconfigured, the leaf-to-WAN reachability tests would fail. 

% But as good as this test suite appears, it has a major testing gap. The policy clause on Lines 8-9, which dictates what happens if the WAN announces a prefix in the internal address space, is untested. As it happens, there is a bug on Line 9---it should say \code{deny} instead of \code{permit}. 

% % B1 has an import policy \code{wan-to-b1} to control which routing messages are accepted from the WAN. Its first clause (line 7-8) is intended to reject routes with destination prefixes that overlap with the data center's internal address space, but it fails to do so because of a typo (line 8 should be \code{deny}). This bug is missed because the test suite is not testing this line. When the WAN is not announcing a prefix within 10.1.0.0/16, the misconfigured clause does not get exercised (and none of the tests fails). 

% This bug is latent but highly serious. As long as W2 does not announce an internal prefix, it does not get triggered. But if W2 (which can send arbitrary announcements) were to start announcing an internal prefix (e.g., 10.1.3.0/24), some or all traffic for data center applications that use that address space will start going toward W2. This redirection will cause an outage for impacted applications, and it also represents a security issue if the traffic is sensitive.

% % How can network engineers systematically discover such testing gaps and prevent outages? 
% % %
% % Manual analysis is infeasible because the relationship between tested network behaviors and configuration elements is complex.
% % %, not to mention the difficulty of reasoning about all possible route announcements that neighbors might generate.
% % %
% % We thus argue for a configuration test coverage tool that can reveal testing gaps as well as quantify the coverage of test suites. As in the software domain, an effective coverage tool will help engineers develop test suites with fewer blind spots and stronger assurance. 

% To find such bugs, we  argue for a test coverage tool for network configuration that can reveal testing gaps and quantify the coverage of test suites. As for software, such a tool will help engineers develop test suites with fewer testing gaps and provide stronger correctness assurance.

% %\brief{We have data plane coverage but it is not enough}

% Our goal of computing configuration coverage is different from data plane coverage~\cite{yardstick}. High data plane coverage does not imply high configuration coverage. In our example, unless W2 were already sending bad announcements, the data plane state is not buggy and even 100\% coverage of it would not reveal the bug. We want to find testing gaps, not in data plane state, but in configuration, which can reveal both bugs that have already impacted the data plane state and latent bugs triggered by different routing messages or failures.

% % metrics that model how well different data plane components such as devices, interfaces, and routes are exercised by data plane tests. However given the difference in control plane and data plane verification, we can not simply reuse data plane metrics. The reason is two-fold.

% %Data plane coverage cannot do this job because they are agnostic about config lines. With control plane tests added to the test suite, it is not enough to have data plane coverage metrics for judging test quality:

% %\begin{enumerate}
%     %\item Some control plane tests check the correctness of the control plane by checking its output (ie, data plane). While data plane plane metrics can be used to judge how much of the output is tested, a major leak is that they fail to reflect which parts of the control plane itself are or are not covered. 
%     %\item The universe of testable space considered by data plane coverage metrics is a single entire data plane. Control plane tests can exceed this range by exercising more than one data plane.
%     %\item Data plane coverage as defined by prior work does not support negative data plane questions
%     %\item Returned values are much more interpretable 
%     %\item Even 100\% data plane coverage is insufficient for control plane verification, as we will reveal in later sections, part of the control plane can only be exercised with some specific environments

%\end{enumerate}

==> Control-Plane-Coverage [arxiv submission] (4)/sections/casestudy.tex <==
\section{Case Studies} 
\label{sec:deployment}

We present case studies of using \sysname on two disparate networks, one a wide-area backbone and another a datacenter. In each case, using realistic test suites, we show that \sysname provides insight into what is and is not covered and how these insights help improve the test suites. 
%We show that the coverage reported by \sysname can help reveal testing gaps and suggest targeted new tests to improve test quality in real-world settings. 
%Using \sysname, we are the first to quantify the coverage of control plane tests in prior works~\cite{bagpipe}. We show that although researchers have made tremendous progress in building expressive and scalable verification tools, little effort have been made in how to better use these tools  The coverage reported is surprisingly low.

\subsection{Case Study I: The Internet2 backbone}\label{sec:internet2}
%The remaining of the section is organized as follows. In \cref{sec:internet2-overview}, we brief the Internet2 network design. In \cref{sec:internet2-coverage}, we show that existing network tests merely scratched the surface of critical aspects to test for this network. Without coverage, network tester are in danger of leaving important aspects of network being untested without knowing it. In \cref{sec:internet2-testdev}, we demonstrate the use of coverage-guided testing framework.
%We start by showing how bad the network configurations were being tested by prior works. We are not saying that these testing/verification tools are not good. In fact, (they are good). It's just that little attention has been paid on how well these tools were being used towards 
%We show that the coverage report generated by \sysname is informative and easy to understand. It helps identify systematic testing gaps--a challenging task even for those who are familiar with the network design. We also show that test quality can be effectively improved with the feedback from \sysname in developing new tests. 
%Finally in 6.4, we compare configuration coverage and data plane coverage metrics under the same network and test suite settings. We show that configuration coverage not only supports more test types but also reveals more testing gaps.

%\subsubsection{Network Overview}
\label{sec:internet2-overview}

Internet2 is a nation-wide network that connects over 60,000 US educational, research and government institutions. The routing design of Internet2 is typical of backbone networks. It has 10 BGP routers spread across the country. The routers are organized as a single autonomous system (AS), and they establish iBGP full mesh on top of internal reachability provided by the IS-IS protocol. The Internet2 routers connect to 279 external BGP peers, and heavily use route import and export policies. The import policy for an external peer has multiple policy statements, some specific to the peer and some shared within the same peer group. Peer-specific policies tend to specify a list of allowed prefixes from this peer, and others are used for sanity checking, preference setting, etc. Export policies are similarly structured. 

Internet2's configurations that we study have 96,672 lines (in Juniper's JunOS format) across all routers. Of these, \sysname's coverage computation considers 64,886 lines. The bulk of the unconsidered lines correspond to device management, IPv6, and IS-IS protocol.
%We also find that 18,085 lines are for "dead code" that will never be exercised. They include defined BGP peer groups with no members and defined routing policies that are never used for any peer. We report such trivially uncovered lines to users separately and compute coverage only for reachable lines. There are 46,801 reachable lines in Internet2. 

%of configurations on the 10 Internet2 routers, including all IPv4 BGP configurations, routing policies, prefix lists, and interface declarations, etc. \sysname reports 47,339 lines of reachable configurations and 24,613 lines of unreachable configurations.
%This set corresponds to the second circle (from outside to inside) in Figure~\ref{fig:overall_measures}. We consider it to be the scope of overall test coverage and testing gap. %\ratul{modeling gap can perhaps be mentioned in the network overview section itself, and not here when it is time to discuss results.} 
 %Based on the taxonomy above, we define the \textit{testing gap} as lines that are reachable but not covered (the set between the third and the fourth circle in Figure~\ref{fig:overall_measures}).

%Within modeled lines, \sysname further classify lines as reachable or unreachable. The \textit{unreachable configurations} can never contribute in producing any data plane facts under any environments. These might be an empty BGP group configurations with no peer in it, or a redundant routing policy defined but never used. While not being testable by data plane tests, some of the unreachable configurations can be tested by control plane tests. For example, an unused routing policy can be directly tested by \code{testRoutePolicy}. However, unreachable configurations do not affect routing anyways, and thus we deem it as out of scope for testing. Figure~\ref{fig:overall_measures} shows an Euler diagram of the concepts of modeled lines, reachable lines and covered lines.

We do not have the data plane state of Internet2, which is needed to run data plane tests. We approximate it using Route Views~\cite{routeviews}, a repository of BGP routes from over two hundreds ASes worldwide. 
%
This data helps approximate BGP messages that external peers of Internet2 send to it. Consider a peer with AS number $X$. If we find a prefix $P$ in RouteViews with AS-path $[A, X, Y]$, we assume that the peer sends $P$ to Internet2 with AS-path $[X, Y]$. The existence of AS-path $[A, X, Y]$ means that AS $A$ must have a route to $P$ with AS-path $[X, Y]$, which it announces to its neighbors. If we find multiple AS-paths for a prefix, we pick the one where $X$ is closest to the origin AS (the last entry in the path). 
%

We use these BGP messages that each peer sends to Internet2 as inputs to simulate Internet2's control plane using Batfish. The data plane state produced by this simulation is a coarse approximation of the real version, but it suffices to meet our goals of running data plane tests and characterizing configuration coverage. 

\subsubsection{Test suite coverage}\ \\
\label{sec:internet2-coverage}

To study how \sysname analyzes coverage for realistic test suites, we use the test suite proposed in Bagpipe~\cite{bagpipe}. It has three tests to validate Internet2's BGP configuration.
%\footnote{We slightly misuse the term test to indicate not only tests in the context of network testing, but also specifications in the context of network verification.}

\newcommand{\BTE}{\textit{BlockToExternal}\xspace} 
\newcommand{\NM}{\textit{NoMartian}\xspace}
\newcommand{\RP}{\textit{RoutePreference}\xspace}
\newcommand{\SANITY}{\textit{SanityIn}\xspace}
\newcommand{\IFREACH}{\textit{InterfaceReachablility}\xspace}
\newcommand{\PSR}{\textit{PeerSpecificRoute}\xspace}
\begin{itemize}[itemsep=0pt]
    \item \BTE: ensure that BGP routes with BTE community are not announced to any external (eBGP) peer.
    \item \NM: ensure that incoming BGP messages from external peers for prefixes in the private address space ("Martian") are rejected.
    \item \RP: ensure that if multiple routes to the same prefix are accepted from multiple external neighbors, the selected route belongs to the most preferred neighbor. The neighbor's preference depends on commercial relationship~\cite{gao-rexford}.  \textit{Customers} are most preferred, followed by {\textit peers}, and then \textit{providers}.
\end{itemize}

We implemented these tests using Batfish. \BTE and \NM are control plane tests. \BTE evaluates all BGP export policies on a set of BGP routes carrying the BTE community and asserts that the result be rejection. We generate the test cases by sampling BGP routes from the data plane state and attaching the BTE community to them. \NM evaluates all BGP import policies on a set of BGP routes destined for Martian addresses and asserts that the results be rejection. \RP is a data plane test. It focuses on destination prefixes available via multiple neighbors and asserts that their local preferences reflect commercial relationship. We use CAIDA data~\cite{caida} to infer commercial relationship between Internet2 and its BGP neighbors.

After running this test suite on Internet2, we find that it covers only 26.1\% of configuration lines across all devices. Only a tiny fraction of configuration lines (0.5\%) are weakly covered, so we do not separate weak/strong  coverage for this case study; we will do that in the next one. 

%Network engineers who find this coverage low would want to better understand what is not covered. 
To help understand what is and is not covered in more detail, \sysname enables network engineers to look at the data from multiple perspectives.
%
\Cref{fig:screenshot_aggregate} shows per-device coverage. We see notable variation across devices, from 11.8\% to 40.5\%. As we show below, the test suite has systematic gaps, and the cross-device variation stems from different devices having different fractions of covered configuration elements. 

\Cref{fig:coverage-original-tests} shows the coverage broken down by the type of configuration elements. For simplicity, we create four buckets of element types, as shown in the legend. The bottom bar shows the fraction of reachable configuration lines in each bucket. The "Test Suite" bar shows the covered fraction of those lines, and the top three bars show the coverage of individual tests. The total coverage of individual tests is $0.6$\%, $0.9$\% and $24.7$\% respectively. \BTE and \NM cover only one type of configuration element (routing policies), and even within this type, they cover a small fraction. \RP covered all four buckets but its overall coverage is still limited.

Finally, \sysname reports that 27.9\% of configuration lines are "dead code" that will never be exercised. They include defined BGP peer groups with no members and defined routing policies that are never used for any peer.\footnote{Per best practices, these lines should be deleted. Or, at a minimum, they should be tested lest someone start using an unused, erroneous policy. When it comes to testing, such lines can never be exercised by data plane tests, though control plane tests may be written for them. }


With 69\% of BGP configurations,  85\% of interfaces,  88\%  of routing policies, and  57\%  of route attribute match lists being completely untested, this test suite is clearly under-testing the network. This leaves the network vulnerable to bugs in untested configurations elements. Prior to \sysname, it was not possible for network engineers to get any insight into the quality of their test suite. It was also not possible for them to get help toward systematically improving tests. We demonstrate this test suite improvement process next.

%To make it worse, network testers can hardly realise this situation without any tool to provide feedback on what aspects of the network has/has not been tested. We therefore argue that this result shows a compelling need of tools of this kind to provide coverage feedback in the practice of network testing and verification.

\subsubsection{Coverage-guided test development}\label{sec:internet2-testdev}
%\xieyang{May need to brief test results (e.g. how many violations are reported). Coverage makes more sense when all tests have passed.}

%Understanding test quality without feedback from coverage is difficult, especially for networks of this level of complexity.

%\sysname helps understand the test quality at three different levels of details. First, at a high level, it quantifies test coverage and testing gaps with two numbers--overall percentage of lines covered by the current test suite and lines that are reachable but remain uncovered. Second, it breaks down coverage statistics into categories and zooms in to user-defined scope of interest. Coverage statistics at this level allow users to identify systematic testing gaps such as a specific BGP group being completely untested, or a specific type of configuration elements being under-covered. Third, it visualizes a line-by-line coverage result as annotations on source configurations. It helps understand detailed testing gaps.
%Next, We demonstrate our study of the Bagpipe test suite on Internet2, using these feedback.
%We demonstrate the value of \sysname by showing that \textit{i)} it helps understand the quality of existing tests and \textit{ii)} it 
\sysname's feedback enables a test suite development process that enables users to systematically improve coverage, which helps test more critical aspects of the network and prevent outages. This process is iterative. In each iteration the user first identifies specific testing gaps and then creates new tests to target those gaps. We demonstrate the process using three iterations that focus on different types of gaps.

%\para{Overall test coverage and testing gap} 
%The overall test coverage of this initial test suite is 30\%, as reported by \sysname. It means that coverage is poor because 70\% of reachable configurations remain completely untested. Figure~\ref{fig:coverage-original-tests} shows the coverage results of each individual test. We break results by configuration element types and plot the coverage for four major types.


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/original_test_suite.pdf}
    \vspace{-10pt}
    \caption{Coverage of the initial test suite broken down to each individual test and configuration type. }
    \label{fig:coverage-original-tests}
\end{figure}

\para{Iteration 1}
We saw that routing policy coverage of \NM test is low (\Cref{fig:coverage-original-tests}) despite that it checks the import policies for all external peers. 
%We doubted that our test implementation might be wrong at first, which can be verified by looking at the line-level coverage and locating lines that have been covered by the test. It turned out that both our test implementation and coverage result were correct. 
To investigate, we look at the structure of Internet2 import policies and find that routers have a policy named \code{SANITY-IN} which is shared by the majority of external neighbors. \Cref{fig:screenshot_lcov} shows this policy with annotated coverage. Each router has an independent copy of this policy, but the copies and the coverage results are identical across routers. Of the five clauses in the policy, the clause \code{block-martians} starting at line 6,896 is the only clause that is covered. %This result instantly helped the user--a student author of this paper--understand how the test worked and get more confidence on the test quality, despite that he or she is not familiar with the design of Internet2 network.
This coverage result confirms that the \NM test did its job, and more importantly, it revealed a systematic testing gap--the other four classes of forbidden routes are not being tested.

Once we know the gap, the solution suggests itself. We added a new test, \SANITY, to enforce that the other four classes of received BGP messages should be rejected. 
%These classes corresponds to the four untested clauses in \Cref{fig:screenshot_lcov} respectively. 
After adding this test, we used \sysname to confirm that this testing gap had been addressed. Routing policy coverage was improved by 0.6\% and all five terms of \code{SANITY-IN} were covered by the new test suite. 
%
The quantitative improvement is low because \code{SANITY-IN} is just one of many policies in the network. With feedback from \sysname, network engineers can identify testing gaps in other routing policies and add more tests in a similar way.\footnote{Automatic test generation based on coverage feedback will further help engineers. We will investigate this in the future.}

%Given the complexity of Internet2 routing policies (with over 4,000 policy terms spanning across over 20,000 lines), the labor of human oversight required to fully understand all testing gaps is still a concern. Computational automation of such process is possible, such as coverage-guided fuzzing, yet is out of scope of this paper.%The details of this testing gap is out of scope of this work, given that Internet2 has over 4,000 policy terms.


\para{Iteration 2}
BGP peer configuration coverage of \RP test in \Cref{fig:coverage-original-tests} is surprisingly low, given that all external BGP peers are supposed to be checked. Upon further investigation we find that the uncovered peers have permitted prefix-lists that do not overlap with other peers' lists, which left these peers untested.

%This surprising number suggests further investigation with finer-grained coverage. As shown in Figure~\ref{fig:bgpgroup}, we break down BGP peer configuration into four different groups and plot the number of covered lines in each group along with total lines in the group. We find that the two BGP groups that this test cares about, one for customers and one for peering-networks, are covered by 50\% and 40\% respectively. This result reveals a testing gap unexpected by test developers. With some further investigation, we find the root cause to be that the allowed prefixes of some external peers does not overlap with others. The \RP test works by comparing local preference attributes, so no route from these peers are tested. This testing gap makes the network vulnerable to latent bugs in these untested BGP peer configurations.

We added a new test, \PSR, to check that BGP announcements received from external peers should be accepted if their prefixes is in a peer-specific prefix list. This test improved 
%overall configuration coverage by 18\%. %and 
BGP peer coverage from 32\% to 46\%. The rest of untested BGP peers are either not allowed to send BGP routes to Internet2 or is intended for other internal use, such as monitoring and management. This test also improved prefix-list coverage from 45\% to 63\%. The remaining of untested prefix-lists are mostly (30\% out of 37\%) ones that are defined by never referenced.

%The routing policy coverage of \RP test is also affected by the previous testing gap. That being said, the coverage at 7\% is still lower than expected. We find a serious flaw of our test implementation when investigating into this gap. As we read the Internet2 configurations,  we found that BGP peers within a same BGP group tend to share a common preference setting policy. And as we checked the coverage of such policies, we noticed a pattern of unexpected low coverage. An example of preference setting policy is shown in Figure~\ref{fig:setpref} with annotated coverage. It was a pattern that all these policies only had their last single term covered. Given this testing gap, it is straightforward to find the root cause. Internet2 and its peers use proprietary communities, such as \code{HIGH-PEERS} on line 12,344, to coordinate route preferences. The external route announcements used by our test did not have any of these communities, therefore the non-default policy terms such as line 12,343 to 12,365 in Figure~\ref{fig:setpref} cannot be tested under the current environment. With feedback from \sysname, we should be able to identify testing gaps related with other untested routing policies in a similar way. Given the complexity of Internet2 routing policies (with over 4,000 policy terms), the labor of human oversight required to fully understand all testing gaps is still a concern. Computational automation of such process is possible, such as coverage-guided fuzzing, yet is out of scope of this paper.%The details of this testing gap is out of scope of this work, given that Internet2 has over 4,000 policy terms.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/bgp_group.pdf}
%     \caption{BGP peer configuration coverage of \RP test broken down to BGP group. \todo{To be updated}}
%     \label{fig:bgpgroup}
% \end{figure}

\para{Iteration 3}
The low coverage of interface configuration in \Cref{fig:coverage-original-tests} reveals another testing gap. \RP is the only test in the initial test suite that checks interface configurations, and it only considers one category of interfaces--ones that are used to establish the tested BGP edges. %The problem is that only external-facing interfaces are being tested, while the majority of interfaces are internal-facing.
Many other interfaces remain untested, including but not limited to ones that associate with untested BGP edges and other routing protocols, and the ones that are unused.


We added a new PingMesh-style~\cite{pingmesh} test, \IFREACH, to check that the IPv4 addresses assigned to interfaces should be reachable from each router in the network. This test increased interface coverage from 15\% to 53\%. The rest of untested interfaces do not have IPv4 addresses assigned.


\Cref{fig:progression} summarizes the coverage improvement for the three iterations of test improvement in our study. After only three iterations, the overall coverage was improved from 26\% to 43\%. 
%
This final coverage number is far from perfect, but our goal was not to develop the ideal test suite for Internet2; we wanted to  demonstrate how coverage information helps develop new tests. 
Networks are complex and we should not expect to get the job done with 6 tests. Many more tests are likely needed. With \sysname, network engineers now have a tool to develop new tests that meaningfully improve coverage.

%We have shown that coverage-guided testing framework can be used to effectively create new tests that improve coverage. We note that the derived test suite is by no means close to a high-coverage test suite. Networks are complex and we should not expect to get the job done with 6 tests. Similar to the road taken by software testing, improving test quality for networks will be a long journey.


%\para{Broken-down coverage statistics} 
%The overall coverage and testing gaps can be broken down in many ways to study test quality among certain aspects of the configuration. We demonstrate two examples that help us identify systematic testing gaps here.
%Figure~\ref{fig:brokendown} shows the coverage and testing gap broken down by configuration element types.
%We find that a large fraction of BGP peer configuration remains in testing gap despite that \RP test is supposed to test all external BGP peers. This surprising number suggests further investigation into this category of configuration, and we will show that in the next example. This chart also shows that the current test suite has low coverage on interface configurations. This number indicates that a significant fraction of network topology is being neglected by the current test suite, which is also surprising given that the \RP tests is supposed to cover physical links used to carry BGP traffic. We also find that the coverage of prefix lists are decent, while the coverage of routing policy is poor. We will use line-by-line coverage visualization to understand testing gaps in these categories later.

%Figure \ref{fig:brokendown} shows the coverage statistics reported by \sysname. The coverage of three individual tests are shown on the left. The covered lines are classified into five categories according to configuration types, shown in different colors. We find that the \BTE and \NM test have very limited coverage. It is as expected because these two tests target very specific routing logic that are related with only a small proportion of configurations.







%\para{Line-by-line coverage visualization} The visualization enables a detailed view of coverage for certain areas of configurations. It is useful for example, when developing a test for a specific routing policy or when further investigation into a specific category is necessary given the results of broken-down coverage statistics.
%In addition to statistical coverage result in percentage, \sysname provides two other useful information to help understand the part of configurations that remain uncovered.

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{figures/setpref.png}
%    \caption{Annotated coverage of \RP test.}
%    \label{fig:setpref}
%\end{figure}



% Coverage results is impacted by how the test is implemented, which is a shared shortcoming with code coverage.



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/improvement_summary.pdf}
    \vspace{-10pt}
    \caption{Coverage improvement with test suite iterations.}
    \label{fig:progression}
\end{figure}

\subsection{Case study II: Datacenter networks}\label{sec:dc}
%We generate synthetic fat-tree \cite{fattree} networks of different sizes by varying the topology parameter $k$ between 4 and 16, which generate networks of up to 320 routers. 
We study the coverage for data center networks which have a different topology and routing design. We create synthetic fat-tree\cite{fattree} networks with routers across three tiers. The leaf routers at the bottom tier connect to hosts. Aggregation routers at the middle tier connect to leaf routers in a pod and to spine routers at the top tier. The spine routers connect to the wide area network (WAN). The WAN is not part of the tested network. %The routing design of these synthetic networks follows RFC7938 \cite{xx}. 
Each leaf router is assigned a /24 prefix which is advertised inside the data center through eBGP. Spine routers receive a default route (prefix 0.0.0.0/0) from WAN via eBGP and propagate it to lower tiers. At each spine router, the entire address space of the network is summarized into a /8 prefix and is announced to WAN. Multipath routing (ECMP) is enabled with maximum number of paths set to 4. Routing policies are only configured at spine routers to white-list the default route received from WAN peers. We synthesize the configurations of these networks in Cisco IOS format.

We study a test suite of three tests inspired in prior works on data center network validation~\cite{rcdc,pingmesh}.

\newcommand{\DRC}{\textit{DefaultRouteCheck}\xspace} 
\newcommand{\PM}{\textit{ToRPingmesh}\xspace}
\newcommand{\EA}{\textit{ExportAggregate}\xspace}
\begin{itemize}[itemsep=0pt]
    \item \DRC: ensure that each router has the default route.
    \item \PM: ensure that each leaf router's assigned subnet is reachable from all other leaf routers.
    \item \EA: ensure that each spine router exports the aggregate route to WAN.
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/fattree_original_test_suite.pdf}
    \vspace{-10pt}
    \caption{Coverage of synthetic datacenter network broken down to each individual test and configuration type.}
    \label{fig:fattree-coverage-original-tests}
\end{figure}
\Cref{fig:fattree-coverage-original-tests} shows the coverage result when the network has a total of 80 routers. Given the uniformity of the network and the test suite, coverage results are similar for other network sizes.
%
The total coverage of individual tests is $81.5$\%, $82.1$\% and $80.7$\%  respectively, and the three tests together cover $85.3$\% of configuration lines. We find that these tests cover largely the same configuration elements---interfaces and BGP peerings between the data center routers---despite checking for seemingly different network behaviors. This result indicates that seemingly distinct network tests can be redundant in terms of configuration testing. 

The coverage of \EA shows a large proportion of weak coverage. This is because a spine router has routes to all leaf routers, so that all leaf subnets contribute to the tested aggregate route, albeit weakly. Separating out weak coverage here avoids false negatives of testing gaps---the aggregate routes would be there even if some of the BGP peering or interfaces are misconfigured, therefore testing the aggregate routes provides a weaker endorsement for the covered BGP peerings and interfaces to be bug-free.

By looking at uncovered configuration lines reported by \sysname, we learn that most correspond to host-facing interfaces on leaf routers.  Adding tests that target those interfaces improves this test suite and eliminate testing gaps. We omit results of this iteration.

==> Control-Plane-Coverage [arxiv submission] (4)/sections/conclusion.tex <==
\section{Summary}
\sysname is a tool that analyzes which configuration lines are tested by a suite of network tests. It uses an information flow model based on control plane semantics to track which configuration lines contribute to tested data plane state. It accounts for non-local and non-deterministic contributions, and for performance, it discovers the graph lazily. Our experiments showed that \sysname successfully reveals coverage gaps for real-world networks and test suites, and these tests can have surprisingly low coverage, e.g., 26\% of configuration lines for Internet2. They also showed how its feedback helps improve coverage.



This work does not raise any ethical issues.

==> Control-Plane-Coverage [arxiv submission] (4)/sections/design.tex <==
\section{Design of \sysname}

\sysname takes as input configuration files, data plane state (protocol RIBs, main RIB and active routing edges) of the network. The data plane state may be pulled from live network or produced by a control plane analysis tools~\cite{cbgp,batfish,hoyan}. In addition, \sysname takes as input what is tested: data plane entries that are tested by data plane tests, and configuration elements that are tested by control plane tests.
This information is produced by network testing tools~\cite{yardstick,batfish}. 

Based on these inputs, \sysname computes which configuration elements are covered.
%It also produces aggregate statistics such as covered fraction of lines or covered fraction of elements of a certain type (e.g., routing policies). 
The core of this computation efficiently mapping a data plane fact to configuration elements that contribute to it. We describe this computation next. 

%The rest of the section is organized as follows. In Section~\ref{sec:ifg} we define IFG--a graph-based intermediate representation that captures information flow between configuration elements and data plane states. Then in Section~\ref{sec:lazyconstruction}, we describe the backward-forward inference framework that allows \sysname to materialize the IFG on demand. Finally, we handle non-determinism of IFG dependencies in Section~\ref{sec:weak_coverage} and discuss potential model extensions in \ref{xx}.

\subsection{Information flow model}\label{sec:ifg}

%\begin{figure}[t!]
%\begin{align*}
%&C \tag*{Configuration elements}\\
%&S = {R \cup F \cup A} \tag*{Data plane state}\\
%&\ \ \ \ R \tag*{RIB entries}\\
%&\ \ \ \ F \tag*{FIB entries}\\
%&\ \ \ \ A \tag*{ACL entries}\\
%&E \tag*{Edges between routing protocol instances}\\
%&M \tag*{Routing messages} \\
%&P \tag*{Paths of routing edges} \\
%\end{align*}
%     \caption{Fact types in information flow graph.}
%     \label{fig:model-entities}
%\end{figure}




IFGs are directed acyclic graphs whose nodes denote network \textit{facts} and edges denote information flow between facts. %An IFG captures the information flow in the stable state of the network.
\autoref{fig:model} shows the types of network facts modeled by \sysname and the information flow between different types.

%\para{Network facts} 
Our model has thee types of facts: configuration elements, data plane state, and auxiliary facts. Data plane state has three subtypes: main RIB entries, protocol RIB entries, and access control list (ACL) entries. 
%
%across all VRFs (virtual routing and forwarding) of all devices,\footnote{VRFs are virtual routers within in a device. Each interface and routing protocol instance belongs for exactly one VRF, and there is one FIB per VRF. Routing information can flow across VRFs using explicit configuration.} 
%
Auxiliary facts help concisely capture information flow dependencies from configurations to data plane state. They have three subtypes: routing edges, routing messages, and paths that carry routing messages. Routing message facts represent messages between routing protocol instances across devices as well as within a device, i.e., redistribution~\cite{redistribution}. This uniform treatment is a modeling convenience. In reality, explicit messages are not exchanged during redistribution (though redistribution is subject to routing policies akin to messages between cross-device routing instances). 
%\brief{This inference framework is general and allows for different definitions of configuration elements. Certain types of configuration objects may be completely ignored or considered at coarse granularity. For instance, an import policy may be considered as one element (covered or not as a whole), or decomposed into its multiple elements, one for each policy clause. }

%\para{The information flow}
%The third is a "disjunction" fact that captures uncertainty in information flow. We describe it in more detail later.
The last column of \autoref{fig:model} shows how information flows among different types of facts. A main RIB entry stems from a protocol RIB entry and optionally another main RIB entry (when its next hop is an IP address whose corresponding output interface needs further resolution). A protocol RIB fact stems from a routing message (for protocols such as BGP), a configuration element (for connected interfaces and static routes), a main RIB entry accompanied with a configuration element (such as when a BGP network statement populates a main RIB entry into BGP RIB) or a set of RIB entries  accompanied with a configuration element (for aggregate routes). ACLs facts stem from configuration facts and have no other dependencies. Routing messages stem from a RIB fact or another message (e.g., post-import-policy message depends on pre-import-policy message), and they also depend on routing edges and routing policy configurations. Inter-device routing edges stem from paths that enable sessions to be established and configuration facts that define peerings; Intra-device routing edges stem from configuration facts that define redistribution. Finally, path facts depends on main RIB facts and ACL facts that impact routing traffic along the way. 
%\ratul{delete everything that follows in this para? it is too detailed a point for most readers.}
%Conceptually, routing messages also directly depend on paths, in addition to the indirect dependency via $m_i \leftarrow e_l \leftarrow \{p\}$. Due to that all messages for a routing edge traverse the same path and are impacted by the same FIB and ACL entries, we omit the edges between messages and paths for our model to be concise.

\begin{table}[t!]
\begin{tabular}{lll}
\toprule
\multicolumn{2}{l}{\textbf{Network fact} } & \textbf{Information flow} 
\\ \midrule
\multicolumn{2}{l}{Configuration element ($c$)}  & None 
\\ \midrule
%\multicolumn{4}{l}{\textbf{Data plane state facts}} \\ \hline \hline
\multirow{7}{19pt}{Data plane state}
& Main RIB entry ($f$) & \makecell[cl]{$f_i \leftarrow r_j$ \\ $f_i \leftarrow r_j, f_k$}
\\ \cmidrule{2-3}
& Protocol RIB entry ($r$) & \makecell[cl]{$r_i \leftarrow m_j$ \\ $r_i \leftarrow c_j$ \\ $r_i \leftarrow f_j,c_k $ \\ $r_i \leftarrow \{r_{j_1}, ...\}, c_k$}
%& A RIB fact stems from one or more of a FIB fact, a routing message, and a set of configuration facts 
\\ \cmidrule{2-3}
& ACL entry ($a$) & $a_i \leftarrow \{c_{i_1}, ... \}$ 
%&  An ACL fact stems from  a set of configuration facts 
\\  \midrule
%\multicolumn{4}{l}{\textbf{Auxiliary facts}} \\ \hline \hline
\multirow{5}{19pt}{Aux-iliary}
& Routing message ($m$) & \makecell[cl]{$m_i \leftarrow r_j, e_k, \{c_{l_1}, ... \}$ \\ $m_i \leftarrow m_j, e_k, \{c_{l_1}, ... \}$ }
%& A message fact stems from  a RIB fact or another message, a routing edge, and a set of configuration facts
\\ \cmidrule{2-3}
& Routing edge ($e$) & \makecell[cl]{$e_i \leftarrow \{c_{j_1},... \}$  \\ $e_i \leftarrow \{c_{j_1},... \}, \{p _{k_1},... \}$ }
%& An edge fact stems from path facts and configuration facts 
\\ \cmidrule{2-3}
& Path ($p$) & $p_i \leftarrow \{f_{j_1}, ...\}, \{a_{k_1}, ...\}$ 
%& A path fact stems from FIB and ACL facts \\ \hline
%\\ \cline{2-4}
%& Policy evaluation & $(c_i,r_j)$ & $(c_i,r_j) \leftarrow c_i,\ [(c_k,r_j)]$ 
%& A path fact stems from FIB and ACL facts \\ \hline
\\ \bottomrule
\end{tabular}
\caption{Information flow model: Types of facts and all possible dependencies for each type. $\{t,...\}$ denotes a set of facts. }
\label{fig:model}
\end{table}


\subsection{Inferring the IFG on demand}\label{sec:lazyconstruction}

%\ratul{Can this whole para be cut? I am not sure what it is adding}
%The information flow model above enables lazy materialization of the IFG. Given a network fact, the model dictates all its immediate parents in the information flow. When applied recursively, all ancestors that lead to the given network fact can be discovered, which enables \sysname to efficiently identify configuration facts that led to tested data plane facts.

Based on the information flow model, \sysname uses a backward-forward inference framework to lazily materialize the IFG from any set of facts whose coverage need to be tracked. The framework can be abstracted with a set of \textit{inference rules} and an iterative construction algorithm. Each inference rule is function that takes a materialized IFG node as input and materializes a set of its ancestor nodes as well as the edges the allows the ancestors to reach the input node. These nodes and edges will be merged into the materialized IFG by the construction algorithm. 
The implementation of these functions uses one or both of the \textit{lookup-based inference} and \textit{simulation-based inference}. Let us elaborate.


%A IFG consists of a set of IFG nodes Each IFG node uses a dictionary to represent a concrete network fact, where the keys denote field names and the values denote. Different types of network facts have different data attributes, for example, a BGP RIB entry  These data attributes include a \code{node_type} field indicating the type of the network fact, such as \code{BGP_RIB_ENTRY} for a or \code{BGP_PEER_CONFIGURATION} and a set of other fields associated with Different types of facts have different data attributes.   and Directed edges are pointers to its immediate parents.
%The detailed specification of network fact types and their data attributes modeled by \sysname is listed in Appendix~\ref{xx}.
%\sysname's inference framework leverages two types of \textit{inference rules} to infer the parent facts based on the child. The first type of rules look up parent facts from input. These rules work by, for example, looking up RIB entries (in the input data plane state) used to produce a FIB entry based on the data attributes of the FIB entry. The second type of rules produces parent facts via targeted control plane simulation. These rules produces network facts that are missing from input, such as routing messages. Control plane simulation needs to be done in forward direction, \IE, from a parent to a child. Therefore, when a parent fact requires simulation, we first look up the grandparent and then use it to produce the missing parent.
%The first type of rules infer the parent based on the child. The second type of rules is a slight generalization of the first and infer grandparents. These two types infer purely \textit{backward}. The third type of rules infer the child based on a parent in \textit{forward} direction, and meanwhile discover other parents of the derived child. This type complements the second type to discover the skipped parents between child and grandparents.

%We use three types of inference rules to discover the IFG. The first type of rules infer the parent based on the child. They rules help infer FIB facts from RIB facts and vice versa. The second type of rules is a slight generalization of the first and infer ancestors. They help infer RIB facts from other RIB facts. RIB facts do not connect directly; they are intermediated by  routing messages. The implementation logic of these rules involves is straightforward--it 

\para{Lookup-based inference} %The network control plane computes the network stable state using well-known semantics, by which some network facts are derived from others. Such relationships can be the basis for inferring the parent of a given fact, but derivations are lossy. 
The computation of a control plane is lossy. For instance, while a main RIB entry may be derived from a BGP RIB entry, we cannot infer the complete BGP RIB entry from the main RIB entry because BGP specific attributes (e.g., AS-path) are not preserved in the main RIB.



\begin{figure}
    \centering
 \begin{minted}[breaklines,linenos,fontsize=\small]{python}
def infer_from_main_rib_entry(f, stable_state):
  if not (f is MainRibEntry and f.protocol == 'bgp'):
    return []
  bgp_entry = stable_state.bgp_rib.lookup(
    host=f.host,
    prefix=f.prefix,
    nexthop=f.nexthop,
    status='BEST'
  )
  return [(bgp_entry, f)] 
 \end{minted}
 \vspace{-15pt}
    \caption{Rule to infer BGP RIB entry from main RIB entry.\label{alg:main-from-bgp}}
\end{figure}



To address this challenge, our inference leverages the stable state. 
It first infers a subset of attributes based on control plane semantics. This partial inference provides enough information for us to look up the complete entry in the stable state.

\Cref{alg:main-from-bgp} shows the simplified function to infer the BGP RIB entry that led to a main RIB entry. 
%Lines 2-4 demonstrates the use of lookup-based backward inference.
%Based on control plane semantics, the type of the parent to be looked up is BGP (Line 4), and the data attributes inferred based on the child are specified on Line 5-8. 
%Based on control plane semantics, each routing protocol instance selects the best route candidate for each \py{prefix} and install it to the router's main RIB. The resulted main RIB entry will have the same \py{prefix} and \py{nexthop} as the protocol-wide best route, besides, it will record the source routing protocol as the \py{protocol} attribute. Therefore, 
Based on control plane semantics, if a main RIB entry indicates its source protocol to be BGP, it must have stem from a BGP RIB entry on the same router with the same \code{prefix} and \code{nexthop} attributes (Lines 5-7). Besides, the BGP RIB entry should have been selected as the best route (Line 8). Such information is enough to uniquely identify the parent within the known stable state. The return value (Line 10) is a list of tuples denoting the IFG edges materialized by this rule.

% \para{Lookup-based inference (old)} The network control plane computes the network stable state using well-known semantics, by which some network facts produce some others. Such computation process is invertible due to the information loss, \IE, a child does not have enough information to fully recover its ancestors. For example, a main RIB entry can be modeled as a 5-tuple while a BGP RIB entry is a 7-tuple:
% \begin{minted}[breaklines,fontsize=\small]{python}
% MainRibEntry(host, prefix, nexthop, protocol, admin_dist)
% BgpRibEntry(host, prefix, nexthop, as_path, communities, local_pref, is_best)
% \end{minted}
% Detail description of each data attribute is shown in \autoref{fig:datamodel}. The \code{as_path} and \code{communities} attributes are not kept when the control plane installs a BGP route into the main RIB. %To resolve information loss, backward inference uses the child information to look up the parent from the known stable state.
% To address this challenge, inference rules leverages the stable state from input. 
% It infers as much as possible data attributes of the parent based on domain-specific knowledge, which is often incomplete due to information loss. After that, it looks up entries that matches known data attributes from the stable state.

\para{Simulation-based inference} Lookup-based inference is not enough to materialize the IFG. Some facts are not present in the stable state (e.g., routing messages), and some facts do not contain enough information to uniquely identify their parents. We use local simulations to complement lookup-based inference. But simulations can only be performed in the forward direction, \IE, to compute a fact using simulations, we first need to know its parent. 
%To the interest of lazy materialization, such discovery needs to be based on existing IFG nodes. 
We use a generalized version of lookup-based inference to discover grandparent facts of a known fact, and then use simulations with the grandparents to infer their children (i.e., parents of the original fact).


\begin{figure}
 \begin{minted}[breaklines,linenos,fontsize=\small]{python}
def infer_from_bgp_message(m, stable_state):
  if not (m is BgpMsg and m.is_post_import):
    return []
  bgp_edge = stable_state.bgp_edges.lookup(
    recv_host=m.host
    send_ip=m.nexthop
  )
  origin_entry = stable_state.bgp_rib.lookup(
    host=bgp_edge.send_host,
    prefix=r.prefix,
    status='BEST'
  )
  pre_import_msg, export_clauses = policy_simulation(
    input=origin_entry,
    policy=bgp_edge.export_policy
  )
  _, import_clauses = policy_simulation(
    input=pre_import_msg,
    policy=bgp_edge.import_policy
  )
  return [(pre_import_msg, m), (bgp_edge, m)] +
    [(cl, m) for cl in import_clauses] + 
    [(origin_entry, pre_import_msg), (bgp_edge, pre_import_msg)] +
    [(cl, pre_import_msg) for cl in export_clauses]
 \end{minted}
%
\caption{Rule to infer ancestors of a post-import BGP message.}\label{alg:bgp-message}
\end{figure}

\Cref{alg:bgp-message} shows the simplified inference rule that infers the ancestors of a post-import BGP message. Line 13 demonstrates the use of simulation-based forward inference to compute a missing parent fact on the fly. The two prerequisites to simulate the BGP message--the grandparent BGP RIB entry (\code{origin_entry}) and the BGP edge--are discovered via lookup-based backward inference, on Line 8 and Line 4 respectively. The simulation returns the derived BGP message after applying the routing policy, as well as the policy clauses exercised during the process. The second forward-simulation (Line 17) is to discover the policy clauses that are hit during the import process. The return value includes the inferred IFG edges that connect to the input node \code{m} as well as ones that connect to parent \code{pre_import_msg}. The former corresponds to information flow $m_i \leftarrow m_j, e_k, \{c_{l_1},...\}$ in \Cref{fig:model} and the latter corresponds to $m_i \leftarrow r_j, e_k, \{c_{l_1},...\}$.


\para{IFG construction} Next, we detail IFG materialization using inference rules.
Assume for now that the information flow is deterministic; the next section discusses how we handle non-determinism. 

As shown in \Cref{alg:ifg-materialization}, the IFG initially contains only the nodes representing the tested data plane state facts from the input and does not have any edges (Line 2). It is then iteratively expanded by applying inference rules on existing nodes. In each iteration, all inference rules are applied to the dirty nodes derived from the previous iteration (Line 8). The new nodes and edges inferred during such process are collected and merged (with deduplication) into the IFG (Line 9-14). The computation repeats until no new facts can be derived in an iteration.
\begin{algorithm}[t]
\footnotesize
\DontPrintSemicolon
  \SetKwFunction{BuildIFG}{BuildIFG}
  \SetKwProg{myproc}{Procedure}{}{}
  \KwInput{Initial nodes $\{v_i\}$; Inference rules $\{\phi_i: v \mapsto \{(u_i, v_i)\}\}$;}
  \KwOutput{Materialized IFG $(V, E)$}
  \KwData{Stable state data plane state (main RIB and protocol RIBs);
    Routing edges; Configuration elements;}
  
    \myproc{\BuildIFG{$\{v_i\}$, $\{\phi_i\}$}}
    {
        $V, E \leftarrow \{v_i\}, \varnothing$ \;
        $V' \leftarrow \{v_i\}$ \tcp*{dirty nodes of previous iteration}
        \While{$|V'| > 0$}
        {
            $V'' \leftarrow \varnothing$ \tcp*{dirty nodes of current iteration}
            \ForEach{$c \in V'$}
            {
                \ForEach{$\phi \in \{\phi_i\}$}
                {
                    $E' \leftarrow \phi(c)$ \;
                    \ForEach{$(u_i, v_i) \in E'$}
                    {
                        \If{$u_i \notin V$}
                        {
                            $V \leftarrow V \cup \{u_i\}$,
                            $V'' \leftarrow V'' \cup \{u_i\}$
                        }
                        \If{$v_i \notin V$}
                        {
                            $V \leftarrow V \cup \{v_i\}$,
                            $V'' \leftarrow V'' \cup \{v_i\}$
                        }
                        \lIf{$(u_i, v_i) \notin E$}
                        {
                            $E \leftarrow E \cup \{(u_i, v_i)\}$
                        }
                    }
                }
            }
            $V' \leftarrow V''$\;
        }
        \Return{$(V, E)$}
    }
\caption{IFG lazy materialization}\label{alg:ifg-materialization}
\end{algorithm}





\subsection{Handling uncertainty}\label{sec:weak_coverage} There are situations where it is not certain which stable state facts contributes to a given fact. One such scenario is BGP aggregation, where a prefix (e.g., 10.10.0.0/16) is added to the RIB iff at least one more of its more specific prefixes (e.g., 10.10.1.0/24) is present. When multiple more specifics are present, we do not know which one triggered the aggregate. Another such scenario is when multiple paths are available for a routing edge to be established, which can happen when the network uses multipath routing. Here, we do not know which path is actually used by routing messages.

\begin{figure}
  \centering
  \subfigure[\label{fig:uncertainty-model}]{
    \includegraphics[height=.8in]{figures/uncertainty-model.png}
    }
   \subfigure[\label{fig:weak-coverage}]{
    \includegraphics[height=.9in]{figures/weak-coverage.png}
   }
   \subfigure[\label{fig:bdd-example}]{
    \includegraphics[height=.9in]{figures/bdd-example.png}
   }
   \vspace{-10pt}
    \caption{Modeling uncertainty. (a) BGP aggregate (F1) has two potential contributors. (b) F5 is weakly covered but F6 and F7 are strongly covered. (c) The predicates of IFG nodes.}
    \label{fig:uncertainty}
\end{figure}

We model such uncertainty using {\em disjunctive} nodes in the IFG. This node points to the parent fact (e.g., the aggregated RIB fact) and the multiple contributors to the parent point to this node. See \Cref{fig:uncertainty-model} for an example where a BGP aggregate could be triggered by either of the two more specific prefixes.  When our inference rules encounter uncertainty during IFG materialization, they produce a disjunctive node and attach all contributors to it as children.

When computing coverage, we must account for uncertainty because the notion of coverage is different. Assume in \Cref{fig:uncertainty-model} that F1 was tested. If the uncertainty were not there, and F2 and F3 directly pointed to F1, the configuration elements that led to F2 and F3 would have been critical to the outcome. But with the uncertainty, those configuration elements are not critical. The configuration elements that led to F2 could disappear without impacting F1.

To model such possibilities, we introduce the notion of {\em weak} coverage. A configuration element is weakly covered if it contributes to a tested fact but its contribution is not critical. %
In Figure~\autoref{fig:weak-coverage}, assume that F1 is the tested fact. Here, F5 is weakly covered; F1 can be derived without any contribution from F5 because F3 can be derived via F6, which is enough to derive the disjunctive child of F1. 
%
F6 is strongly covered; without it, neither F2 nor F3 can be derived and thus the disjunctive node cannot be derived. 
%
F7 is also strongly covered because it contributes to F4, which is essential to F1. 

%When considering multiple tested facts, a configuration is weakly covered if it is weakly covered by all tested facts. %In IFG terms, it means that removing the configuration fact, and recursively its parent facts, will ultimately remove some tested fact. During recursive removal the disjunctive node is removed iff all of its children was removed.
%
%In Figure~\autoref{fig:weak-coverage}, assume that F1 is the only tested fact. Here, F5 is weakly covered. Its removal will remove F2, but the disjunctive node is not removed (since F3 is not removed) and thus F1 is not impacted. In contrast, F6 is not weakly covered. Its removal will remove both F2 and F3, thus removing the disjunctive node and then F1. F7 is not weakly covered either because its removal will remove F4 and then F1.

After materializing the IFG, \sysname labels each covered configuration element as strong or weak. The label is determined  
as follows. We first assign a Boolean variable to each configuration element in the IFG. Next, we build a Boolean predicate of each IFG node on top of these variables. The predicate of a fact depends on the predicate of its ancestors in the IFG: A normal node depends on the conjunction of its immediate parents, and a disjunctive node depends on the disjunction of parents. Therefore the predicate of any IFG node is ultimately composed of the variables associated with configuration elements that lead to it, denoted as $\Gamma(v)=F(x_1, \dots, x_n)$. \Cref{fig:bdd-example}
shows the predicates of IFG nodes in \Cref{fig:weak-coverage}. We represent these Boolean predicates using Binary Decision Diagrams (BDDs)~\cite{bdd} and build BDD predicates by traversing the IFG. Once the predicates are built, we test graph reachability and logical necessity between each pair of configuration facts and tested facts. Necessity $\neg x_i \Rightarrow \neg \Gamma(v)$ is equivalent to unsatisfiability of $\neg x_i \wedge \Gamma(v)$. While (un)satisfiability is NP-Complete in general cases, we note that it is efficient in our case---it can be reduced to computing the cofactor $\Gamma(v)|_{x_i=0}$ and testing whether the cofactor is constant false, both of which are efficient using BDD operations.

We further reduce the size of BDD predicates by precluding configuration facts that can reach tested facts via a path with no disjunctive node, such as node F7 in \Cref{fig:weak-coverage}. These configuration facts must be strongly covered so their necessity do not need to be tested. Besides, their validity variables can be replaced with constant true when building BDD predicates, which will not affect the strong/weak classification of other configuration elements. %We prove the soundness of this heuristic in Appendix \ref{xx} \brief{to be added}. 
We empirically find this heuristic to be effective in reducing the number of variables used for weak coverage computation.


%\subsection{Computing coverage from IFG}

%\subsection{Extensions}

%Current modeling has several limitations. First, it models one concrete data plane at a time. Some control plane verification tools are capable of reasoning multiple data planes (under different environments) via semi-symbolic data plane simulation~\cite{houyan}, where data plane states (\EG, RIB tables) contains some symbolic encoding of the environment. \sysname can be extended to support these symbolic data attributes. \brief{IFG can even be extended to be fully symbolic.}

%Second, the current notion of coverage only considers the configuration facts that positively contribute to the tested fact. According to control plane semantics, the presence of a route also depends on the \textit{absence} of more-preferred routes, so that the configurations that negatively contribute to potential better routes (also known as the negative-provenance problem \cite{negativeprovenance}) may need to be considered as (a separate class) of coverage. \sysname can be extended to support the reasoning of negative provenance by modeling "dropped routes" as facts.

%\xieyang{Mutation and negative provenance can also fit in this framework. For negative provenance, we need to model dropped routes or ``non-existance'' of routes. Mutation-based coverage can be modeled as edges from config facts to the facts that will be affected by its mutation, it's hard to compute these edges though.}

%\xieyang{Discuss VRF, prefix-lists, BGP groups, the details of which are not explained in this section}


==> Control-Plane-Coverage [arxiv submission] (4)/sections/eval.tex <==
% \section{Additional Evaluation} \label{sec:evaluation}

% The previous section showed how \sysname helps users understand and improve coverage; in this section, we study its performance and how configuration coverage differs from data plane coverage.

\begin{figure*}
    \centering
    \subfigure[Internet2.\label{fig:time_internet2}]{
    \includegraphics[height=.48\columnwidth]{figures/internet2_performance.pdf}
    }
    \hfill
    \subfigure[Fat-tree networks.\label{fig:time_fattree}]{
    \includegraphics[height=.48\columnwidth]{figures/fattree_performance.pdf}
    }
    \vspace{-10pt}
    \caption{Time to compute coverage.}
    \label{fig:performance}
\end{figure*}

\section{Performance Evaluation}\label{sec:performance}
We benchmark the performance of \sysname on both types of networks we studied above. %\todo{some details on machine hardware and software}. 
Our test machine has two Intel Xeon CPUs (16 core each, 3.1 Ghz), 384 GiB of DRAM, and runs Ubuntu 18.04.


%\para{Internet2 backbone} 
\Cref{fig:time_internet2} shows the time to compute coverage for each test in \cref{sec:internet2} and for the full test suite. It breaks out the time spent on simulations and strong/weak labeling, and, for reference, also shows the test execution time. We see that coverage computation is reasonably fast. The full test suite takes only 99.4 seconds. In comparison, the test execution takes 2,358 seconds. The total coverage computation time is less than the sum for individual tests because facts tested by multiple tests are tracked only once. The graph also shows that simulations and strong/weak labeling are a minority component, which means that most of the time is spent on walking the IFG and doing lookups in stable state for backward inference. 

%\begin{figure}
%    \centering
%    \begin{tabular}{llllll}
%        \toprule
%        \textbf{Test name} & \textbf{Test} & \textbf{Cov.} & \textbf{Back-} & \textbf{For-} & \textbf{Weak} \\ \hline
%        \BTE & 19.6 & 0.14 & 0.08 & 0 & 0.06\\
%        \NM  & 13.2 & 0.29 & 0.19 & 0 & 0.10\\
%        \RP  & 85.3 & 23.4 & 16.1 & 6.94 & 0.36\\
%        \SANITY & 0.67 & 0.07 & 0.04 & 0 & 0.03\\
%        \PSR & 2.62 & 25.8 & 18.3 & 8.5 & 0.97\\
%        \IFREACH & 514 & 10.4 & 9.45 & 0.86 & 0.15 \\
%        Test suite & 635 & 38.4 & 24.1 & 12.7 & 1.62 \\
%        \bottomrule
%\end{tabular}
%    \caption{Performance results on Internet2.}
%    \label{fig:internet2_time}
%\end{figure}




%\para{Synthetic datacenter networks}
%\begin{figure}
%    \subfigure[Comparing coverage computation time to test execution.\label{fig:fattree_overall}]{
%        \includegraphics[width=.9\columnwidth]{figures/fattree_scaling.pdf}}
%    \hfill
%    \subfigure[Breakdown.\label{fig:fattreee_breakdown}]{
%        \includegraphics[width=.9\columnwidth]{figures/fattree_breakdown.pdf}}
%    \subfigure[IFG construction scales linearly to IFG size.\label{fig:fattreee_analytics}]{
%        \includegraphics[width=.9\columnwidth]{figures/fattree_analytics.pdf}}
%    \subfigure[Weak coverage corner cases.\label{fig:fattreee_weak}]{
%        \includegraphics[width=.9\columnwidth]{figures/fattree_weak.pdf}}
%    \caption{Performance results on DC networks.}
%    \label{fig:fattree_scaling}
%\end{figure}
\Cref{fig:time_fattree} shows test execution and coverage computation time for the test suite in \cref{sec:dc}, as a function of the data center network size. Coverage computation takes 4,413 $sec$ on the largest network, which has 2,040,624 RIB entries. This time is less than 9\% of the time to execute the test suite. While substantial, we deem it acceptable in practice. Configuration coverage analysis can be run in the background, as code coverage is often run. \sysname does not slow down test execution, which is on the critical path to finding configuration errors and updating the network.

However, time to compute coverage increases rapidly with network size. This is because the number of RIB entries grows quadratically and so does the number of vertices in the IFG. We find that the average time to materialize an IFG node does not change substantially because all computation is local to the node. The scaling trends suggest that to scale \sysname to much larger networks, we need a concurrent implementation of IFG materialization. Our current implementation is single-threaded (as Python interpreter is single-threaded).

%\ratul{OK to cut this now?}
%We find that the average times to build an IFG node via backward/forward inference converge to stable numbers as the network size grows, which are 0.24 $ms$ and 1.72 $ms$ respectively. In backward inference, most of time is consumed in matching a route with specific fields in routing tables. In forward inference, most of time is consumed in sending policy evaluation questions to Batfish and waiting for the response. Its performance is gated by serialization/deserialization delays.

%During the benchmark we found that BDD weak coverage explodes in extreme cases, such as in the \EA test. We argue that it is not a big concern for most cases. As shown in \ref{fig:fattreee_weak}, time to compute weak coverage for the entire test suite is short, despite it containing the aggregate export test.



\section{Comparison to Data Plane Coverage}\label{sec:dp_vs_cp}
%\brief{Goal 1: 100\% dp coverage cannot cover the entire control plane. Goal 2: test development may be fooled by dp coverage because all tested routes may hit the same subset of configs and thus may not be comprehensive nor efficient. Goal 3: cp coverage is better interpretable and guides the operator to the root cause}
\begin{figure*}[t!]
    \centering
    \subfigure[Internet2.\label{fig:cov_internet2}]{
    \includegraphics[height=.47\columnwidth]{figures/internet2_coverage.pdf}
    }
    \hfill
    \subfigure[Fat-tree with $k$=10.\label{fig:cov_fattree}]{
    \includegraphics[height=.47\columnwidth]{figures/fattree_coverage.pdf}
    }
    \vspace{-10pt}
    \caption{Comparing control plane and data plane coverage.}
    \label{fig:dp_cp}
\end{figure*}

We demonstrate the unique value of control plane coverage by comparing it to data plane coverage. Following Yardstick~\cite{yardstick}, we quantify data plane coverage as the proportion of main RIB (forwarding) rules exercised.  \Cref{fig:dp_cp} shows the comparison for different cases. \Cref{fig:cov_internet2} shows the comparison for Internet2 for all tests in \cref{sec:internet2} and a hypothetical data plane test that inspects all main RIB rules. \Cref{fig:cov_fattree} shows the comparison for fat-tree tests in \cref{sec:dc}.

Besides the obvious advantage that only control plane coverage can support control plane tests---the graphs show 0\% data plane coverage for these tests---there are two main advantages to using control plane coverage to guide network test development.
%
First, it reveals testing gaps that can not be revealed by data plane coverage. Tests with high data plane coverage do not necessarily have high control plane coverage, as we can see in the last row of \Cref{fig:cov_internet2}. Covering 100\% of the data plane state covered only 41\% of the configuration. If the engineers were to improve the test quality under the guidance of only data plane coverage, they would not know that 59\% of the configurations remain untested. The reason of this disagreement is that some configuration lines are only exercised under specific environments (failures, routing messages). For instance, list-filtered route policies apply on BGP messages within a specific range, and will only be exercised when such messages appear in the environment. 

Second, testing more data plane state can sometimes be redundant in covering configurations, when the tests hit the same configuration elements. For example, the \DRC test in \Cref{fig:cov_fattree} has only 1.8\% data plane coverage because it only tests default routes, which is a small fraction of all main RIB routes. However, because correct propagation of default routes incorporates many BGP peerings and interfaces in the network, this test has extensive configuration coverage (87\%). The \PM test covers much more data plane state (88\%), but adding it atop \DRC has little value because this state is derived from almost the same set of configurations lines. %We therefore argue that control plane coverage is more precise in finding testing blind spots in the control plane.
%On the other hand, a test with low data plane coverage can in some cases effectively cover a large portion of configurations. 
We do not necessarily imply that engineers should drop one of these tests, as there may be other reasons to keep both. Our observations are about their value toward configuration coverage. 

%The side-by-side comparison of data plane coverage (rule coverage quantifies the proportion of FIB rules exercised by the test suite and interface coverage reflects the proportion of interfaces used by tested FIB rules for forwarding) and configuration coverage of the four test suites are shown in Figure \ref{fig:dp_cp}.

%\brief{add a plot showing the cdf of dependent lines used to produce a fib rule}

%We thus argue that control plane coverage is a better measure of comprehensiveness in verification of network configurations.

==> Control-Plane-Coverage [arxiv submission] (4)/sections/impl.tex <==
\section{Implementation} \label{sec:implementation}

%\brief{Instead of instrumenting Batfish and reusing some of its data models, we build our tools as a standalone tool and build our own data model outside. We do need more memory space but we get faster development and robustness against Batfish changes}

We implemented \sysname with 4,000 lines of Python code. A total of 18 lambdas (Python functions) encode the IFG inference rules. 
\sysname uses Batfish~\cite{batfish-gh} to extract configuration elements from configuration files and to run targeted simulations, and it uses CUDD \cite{cudd} for BDD operations.

% It computes coverage for networks analyzed Batfish \cite{batfish}, an open-source control plane verification tool that supports all the test types mentioned in Section \ref{sec:background} and has been used in the operation of many real-world networks. Batfish provides a set of Python APIs for its users to supply network configurations as input, retreive derived network state, and run queries of supported test types. We implemented our system as a standalone Python module that can easily be used along with Batfish Python APIs.

\begin{table}\footnotesize
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ll}
\toprule
\textbf{Type} & \textbf{Purpose} \\ \midrule
Interface & Interface and its settings (e.g., addresses) 
%\\ \midrule
%BGP process & Settings of a BGP process (e.g., AS number) 
\\
BGP peer & BGP peer settings (e.g., IP address, AS number)
\\
BGP peer group & BGP peer settings inherited by one or more peers
\\
Route policy clause & One clause in an export or import route policy
\\
Prefix list & List of prefixes, used in route policy clauses
\\
Community list & List of BGP communities for route policy clauses  
\\
AS-path list & List of AS-path expressions for route policy clauses
\\ \bottomrule
\end{tabular}
    \caption{Configuration elements analyzed by \sysname.}
    \label{tbl:config-elements}
\end{table}

\sysname supports all major router vendors supported by Batfish, including Arista, Cisco, and Juniper. It builds a vendor-neutral representation of configuration elements using vendor-specific information provided by Batfish. 
%
Types of configuration elements currently analyzed by \sysname are listed in \autoref{tbl:config-elements}.  
%
%that link these configuration elements to data plane state. 
%Each lambda takes a fact as input and returns one or more derived facts. For backward inference rules, we express their inference logic in generic Python code and their tuple matching using \code{pandas} library. For forward inference rules, we simulate route processing using Batfish \code{testRoutePolicy} API.

% The configuration elements under consideration are interface declarations, BGP configurations, routing policies (also known as route-maps or policy statements), prefix lists, community declarations and as-path declarations. All elements are atomic except BGP configurations and routing policies. An atomic element may consist of multiple lines, and testing any part of it will make the entire element considered covered. For BGP configurations, each peer configuration is considered an atomic element, and the remaining lines inside each peer group configuration, \IE, lines within a peer group that does not belong to any individual peer, is considered an atomic element. For routing policies, each policy term (also known as route-map clause) is atomic, and the remaining lines inside each policy is an atomic element. 

\sysname may not consider all components of a device's configuration. One category of such components device management configuration (e.g., login settings), which does not impact data or control plane functionality. The second category is control plane components that are not currently modeled by \sysname. This includes IPv6 (which is not modeled by Batfish currently) and routing protocols other than BGP (e.g., OSPF). The presence of unconsidered components does not imply that \sysname cannot be used for that network. As we show in the next section, \sysname provides helpful coverage information for parts that are considered.

% \begin{figure}
%     \centering
%     \includegraphics[width=.8\columnwidth]{figures/overall_measures.png}
%     \caption{A taxonomy of configuration lines. The overall test coverage is defined as the ratio of covered lines to reachable lines.}
%     \label{fig:overall_measures}
% \end{figure}





%We collect the input to \sysname in the following way. 1) Retrieve parsed configuration elements from Batfish. Specifically, \code{definedStructures} API reports the name and line numbers of each supported elements, several other configuration property APIs such as \code{bgpPeerConfigurations} and \code{interfaceProporties} report vendor-neutral representation of corresponding elements. 2) Retrieve data plane state from Batfish. We use \code{routes} and \code{bgpRibs} APIs for main RIB and BGP RIB entries, respectively. We then process main RIB to generate FIB entries as they are not directly available from Batfish. \sysname does not model ACLs at the moment. 3) Identify tested data plane entries from the return values of Batfish traceroute and reachability queries. We follow the principles of Yardstick~\cite{yardstick} in this computation. 4) Identify tested policy terms from the return values of Batfish \code{testRoutePolicy} queries, which contains a trace of hit terms during the evaluation of the policy. \xieyang{The forth input would make more sense to be control plane ATU--(policy, input route) pairs}

%For backward inference rules--the first and second types of inferences rules computes an immediate predecessor and a non-immediate ancestor respectively for a given fact--the output fact is derived in two steps. The first step is counterfactual reasoning based on control plane semantics. Each backward lambda 

After constructing the IFG, which yields information on which configuration elements are covered, \sysname computes which lines are covered. Each element typically spans multiple configuration lines, and when an element is covered, it deems all of those lines as covered. 
%In this sense, one may think of a configuration, an element is like a basic block in software, all of whose lines are covered 

Based on element and line coverage, \sysname produces three main outputs. The first is a coverage report at the granularity of individual lines (or elements). We produce this report in the \code{lcov} format, which is supported by common code coverage tools and enables users to visualize coverage results as annotations on configuration files. See  \Cref{fig:screenshot_lcov} for an example. The second is coverage aggregated at the file level, generated with the help of GNU LCOV~\cite{lcov}. See \Cref{fig:screenshot_aggregate} for an example. The third output is coverage aggregated by the type of configuration element, which shows what fraction of elements of each type are covered.

% Two output formats are supported by \sysname, providing both high-level and detailed view of coverage results. The first sort is aggregate coverage results such as the percentage of covered lines over all reachable configurations. This result can be used as a high-level measure of test quality. Aggregate coverage results can also be broken down into different categories such as for individual routers or different types of configuration elements. Broken down coverage results help identify systematic testing gaps when coverage for a specific category is lower than expected. Figure~\ref{fig:screenshot_aggregate} demonstrates aggregate coverage results for an example network with 10 routers. 

These outputs help users uncover testing gaps and improve their test suites in different ways. The aggregate results help identify systematic gaps such as "router A is poorly covered" or "routing policy clauses are poorly covered." The line-level results help them zoom in to specific gaps and develop tests that target them. The case study in the next section demonstrates this test suite improvement process.

\begin{figure}[t]
    \subfigure[Line-level coverage. Green background denotes covered lines, and red denotes uncovered lines. Some lines are collapsed for simplicity.\label{fig:screenshot_lcov}]{
        \includegraphics[width=\columnwidth]{figures/screenshot_nomartian.png}}
    \hfill
    \subfigure[File-level aggregate coverage. The overall coverage is at top right, and the coverage for individual files (devices) is in the table.\label{fig:screenshot_aggregate}]{
        \includegraphics[width=\columnwidth]{figures/screenshot_aggregate.png}}
    \vspace{-15pt}
    \caption{Example \sysname outputs.} \label{fig:screenshot}
\end{figure}


%It takes as input the test results returned by Batfish and translates them into tested facts. It then lazily constructs the (covered subset of) dependency graph that contains all direct and indirect dependencies of tested facts. The graph construction has two phases. In the first phase we retrieve facts that can be reused by making API calls to Batfish. Facts that can be reused include all input facts (configuration blocks modeled by Batfish) and some derived facts (main RIBs, BGP RIBs, BGP session status, \ETC) The missing facts include BGP announcements and behavior facts. In the second phase we iteratively expand the graph to a fixed point by computing the direct parents of existing facts in each step. The computation follows the approach described in Section \ref{sec:lazyconstruction}. The backward mapping is implemented using 16 lambdas, where each lambda knows how to map a fact of a specific type to its direct parents, according to dependency relations defined in Section \ref{sec:dependencyrelations}. We also implemented the computation of both control plane (line coverage) and data plane coverage metrics (rule coverage and interface coverage) from the constructed dependency graph.

%Our system is implemented with zero-instrumentation to Batfish. 

==> Control-Plane-Coverage [arxiv submission] (4)/sections/intro.tex <==
\section{Introduction}
\label{sec:introduction}

%The reliability of networks is critical to the services built on top of them. However, networks are brittle and even a small misconfiguration can take them down. 
As critical infrastructure, networks must be highly reliable but, unfortunately, network outages are quite common. A primary culprit is networks' reliance on complex, low-level commands embedded in their configuration. The configurations dictate how routers select best paths and forward traffic.
%
Day-to-day updates to them is error-prone, leading to outages that knock off important online services (e.g., banking), ground airplanes, and disable critical communication (e.g., emergency calls)~\cite{time-warner,united,twitter,bank, t-mobile}.

%For instance, when apps were taken down by just one faulty command \cite{fboutage}, not only the company paid a heavy price but their billions of users were also disrupted for multiple hours.

To improve network reliability, automatic testing and verification of configurations is becoming commonplace.
%, to find configuration bugs and gain confidence in the correctness of configurations. 
Today, network operators have at their disposal many tools with increasing sophistication that can scale to large networks and check various aspects of network behavior \cite{rcdc,jingjing,hoyan,libra,aws-inspector}. 

However, using such tools is not sufficient by itself; one must also use them \textit{effectively}. Outages can occur despite automated testing when the test suite is poor and does not cover key aspects of network configuration. This was the case with the massive Facebook outage during which Facebook, WhatsApp, Instagram, and Oculus were unavailable for six hours~\cite{fboutage}. 
%
%Facebook's tests did not cover some key configuration lines.
Current tools have pushed the limits of \textit{what can be tested} but left open the question of \textit{what need be tested}. 

Without tool support, it is difficult for engineers to know if they are effectively testing network configurations. 
%They rely on their understanding of network behavior to create tests. 
In industrial networks with hundreds of thousands of lines of configurations, engineers' understanding of network behavior and dependencies is necessarily incomplete. It is even harder to evolve an existing test suite after the network evolves because the engineers likely do not know what the old test suite is or is not testing for the updated network. 

%There is no metric nor system to help network engineers judge how good a test suite is and what it does not test.
Recent work has proposed data plane coverage~\cite{yardstick} to reveal testing gaps. It shows which data plane elements, such as forwarding rules, are exercised by a test suite.
However, well-tested data plane does not imply well-tested configurations.   
% 
Data plane elements are the output of network's configurations (which define its control plane) and the current operating environment (failures, external routing information). 
%Even when data plane coverage is high, configuration coverage can %remain low. And, somewhat paradoxically, the reverse can be true as well. 
%coverage, while in another network, testing 2\% of data plane elements can lead to 83\% configuration coverage.
%However, data plane metrics are insufficient to reveal all configuration bugs and are inaccurate in measuring coverage of configurations. 
%This divergence exists because c
Testing a given data plane only tests configuration elements that  are exercised in that particular environment.
Other configuration elements are not tested. We demonstrate this empirically via a scenario where testing {\em all} data plane elements leaves over half of configuration lines untested.

%Configurations are the network's control plane, and they thus anticipate a wide range of operating environments (failures, external routing information). 
%A given data plane stems from a specific environment and testing it  
%Many kinds of control plane tests fix an operating environment, execute the control plane configuration and then test the resulting data plane. Though the generated data plane may be well tested, other operating environments may generate completely different data planes, and might do so by executing different parts of the control plane configuration. Hence the data plane coverage metrics tell us little about the degree to which we have tested the control plane. 


%These are because a specific data plane is the output of configurations under specific environmental conditions. A specific output is bug-free does not imply that the configurations are bug-free, because some parts of configurations may have not been used to produce this output. Moreover, different data plane elements may be the result of a same collection of configuration elements, and thus testing more of such data plane elements cannot get more configuration elements covered.


We develop \textit{configuration coverage} to provide comprehensive and precise feedback to network engineers on test suite quality. Our goal is to identify exactly which configuration lines are being tested and which ones are not. Further, we want to consider all configuration elements, not only those that contribute to the current data plane. The precise nature of this feedback (untested configuration lines) helps improve tests---add tests that target untested lines---which in turn can improve network reliability. This is similar to how code coverage tools help improve tests and software quality~\cite{google-coverage, vs-coverage, codecov}.

A major challenge we face is that many network tests do not exercise configurations directly. Instead, they reason about the data plane elements produced by configurations. We need to infer the configuration elements that contribute to the a tested data plane element. 
This inference is complicated because contributions can be non-local and non-deterministic. In a distributed control plane, a piece of tested routing information may have been propagated and transformed multiple times along its path, and both local and non-local configurations may have contributed to its existence. For example, the path attributes of a BGP route is shaped by routing policies on each and every hop that it traversed. Further, not all contributions are deterministic. For instance, any one of possibly multiple sub-prefixes can lead to the route of an aggregate prefix. We must scalably account for local and non-local contributions and for non-deterministic contributions.

Our solution is to model the contribution between configuration elements and data plane elements as an \textit{information flow graph}. An IFG is a directed acyclic graph (DAG) where vertices denote network elements and edges denote contributions. In addition to direct contributions from configuration elements to data plane elements, we also model contributions between data plane elements (from predecessors to successors). For instance, a BGP route contributes to the BGP message that derived from it. Indirect contributions are thus modeled by multi-hop paths in the DAG. %We also combine graph structure with logical conjunctions/disjunctions to capture whether contributions are (non-)deterministic.
When contributions exhibit non-determinism, we use special \textit{disjunctive} nodes to organize possible DAG paths that may contribute to a given data plane element.

We build a tool called \sysname based on this model. It annotates which configuration lines and logical elements are tested by a given test suite and produces aggregated coverage statistics.  
%\sysname computes configuration coverage using three inputs, the configurations, a stable data plane state, and the set of network elements\footnote{Both data plane elements and configuration elements are supported for completeness. The coverage computation for the latter is straightforward. An examples of network tests that directly analyze configurations is routing policy evaluation.} that are directly tested. 
To efficiently map tested data plane element to the set of contributing configuration elements, it materializes the IFG lazily, instead of tracking contributions proactively (during data plane generation). This design avoids the cost to compute and store contributions for transient or untested data plane elements. 
%It also makes \sysname agnostic to the data plane generation method, allowing it to support a wider range of network testing and verification tools---data plane states used by different tools can be pulled from running networks\cite{xx}, generated via simulation \cite{xx}, or via emulation \cite{xx}. Finally, by computing coverage offline, \sysname does not require instrumentation of testing tools and it does not slow down test execution.
\sysname is open-sourced on GitHub~\cite{netcov-github}.
%\footnote{For anonymity, we have changed the name of the tool for this submission.}

%\sysname supports configuration syntax for different vendors using a vendor-neutral model of configurations. It also supports a rich (but incomplete) set of configuration features such as interfaces, BGP peering and routing policies. Our implementation of \sysname reports configuration coverage in two easy-to-use formats, namely file-level statistics and line-level results as colored annotations on source configurations. 

%One potential approach to know information flow is to use do a high-fidelity simulation of the entire data plane and carefully trace the contributions in the process. It is non-ideal due to the high instrumentation and run-time overhead. Based on our observation that the static data plane state contains enough information to recover the information flow, we materialize the information flow model lazily. This also allows us to eliminate the cost for transient states and untested states.

We evaluate \sysname on Internet2, a nation-wide backbone network in the USA, and on synthetic data center networks. We show that test suites proposed in prior work can have poor coverage. For instance, we found that the three tests proposed by Bagpipe~\cite{bagpipe} covered only 26\% of the configuration lines of Internet2. 
%
We also show how surfacing untested configuration elements suggests new tests that will improve coverage. By adding just three such tests to the Internet2 test suite based on \sysname's feedback, we could improve coverage to 43\%, and more similar tests can be added to further increase coverage.
%
%We benchmark the performance of \sysname on both realworld and synthetic networks. 
\sysname performs reasonably well. The time to compute coverage is 1.2 hours for the largest network that we study, which has over 2 million forwarding rules. This time is an order of magnitude less than the time to execute tests. 

Stepping back, we note that networking is not alone in its reliance on configuration. Today, a lot of infrastructure and distributed applications are deployed by composing existing components using configuration (e.g., infrastructure deployment using Terraform, and application deployment using containers and service meshes). These  configurations are central to correct behavior, which is why there is an intense focus on testing them properly~\cite{terraform-test, istio-test}. As for networks, there are no tools to help engineers discover how well the configurations are tested. The techniques developed in our work, the IFG-based contribution tracking and its lazy traversal, can provide a starting point toward better testing of infrastructure and distributed application configuration as well.

%Analogous to code coverage in software testing, we analyzes which lines of router configurations are covered or nor covered during the execution of a test suite. The result can be used to quantify the rigorousness of the test suite and help discover the blind spots.

% \section{Introduction (old)}\label{sec:introduction}

% %The reliability of networks is critical to the services built on top of them. However, networks are brittle and even a small misconfiguration can take them down. 
% As a critical infrastructure of the modern world, networks are supposed to be reliable. But unfortunately, networks are brittle because their behavior is governed by complicated low-level commands--also known as network configurations. The day-to-day maintenance of these configurations are error-prone, which have led to frequent and costly outages \cite{}. For instance, when apps were taken down by just one faulty command \cite{fboutage}, not only the company paid a heavy price but their billions of users were also disrupted for multiple hours.

% In light of this, automatic testing and verification have arisen in both the academia and industry to find bugs and gain confidence in the correctness of configurations. Over the last few years, researchers have produced many tools with increasing sophistication that can scale to large networks and check various aspects of network behavior \cite{}. 

% However, as we learnt from helping develop verification for multiple networks, outages can still occur \cite{fboutage} when the tests are incomplete and missed some key aspects of the network. The cause of this problem is twofold. First, network engineers rely on their understandings of network behavior to choose what tests to use. And in today's industrial networks with at least $O(10k)$ lines of configurations, these understanding can hardly be complete. Second, improving an incomplete test suite is difficult, in fact, people may not even know whether a test suite is complete or not. Verification tools have pushed the limits of \textit{what can be tested} but left the question of \textit{what need to be tested}. 

% %There is no metric nor system to help network engineers judge how good a test suite is and what it does not test.
% In response to this challenge, recent study proposed data plane coverage metrics \cite{yardstick} to help judge test quality and reveal testing gaps. These metrics quantify the proportion of data plane elements, such as forwarding rules, that are exercised by a test.
% However, data plane metrics are inaccurate in measuring coverage of configurations. 
% Even when data plane coverage is high, configuration coverage can remain low. And, somewhat paradoxically, the reverse can be true as well. For example, our study (\cref{sec:dp_vs_cp}) show a case where 100\% data plane coverage corresponds to only 56\% configuration coverage, while in another network, testing 2\% of data plane elements can lead to 83\% configuration coverage.
% %However, data plane metrics are insufficient to reveal all configuration bugs and are inaccurate in measuring coverage of configurations. 
% Control plane configurations are complex, as they must anticipate a wide range of operating environments.  Many kinds of control plane tests fix an operating environment, execute the control plane configuration and then test the resulting data plane. Though the generated data plane may be well tested, other operating environments may generate completely different data planes, and might do so by executing different parts of the control plane configuration. Hence the data plane coverage metrics tell us little about the degree to which we have tested the control plane. 


% %These are because a specific data plane is the output of configurations under specific environmental conditions. A specific output is bug-free does not imply that the configurations are bug-free, because some parts of configurations may have not been used to produce this output. Moreover, different data plane elements may be the result of a same collection of configuration elements, and thus testing more of such data plane elements cannot get more configuration elements covered.


% In this work, we present \textit{configuration coverage} to provide comprehensive and precise feedback in developing better network test suites. Configuration coverage evaluates the quality of tests defined as the proportion of configuration lines that are exercised. It considers all configuration elements instead of only the ones that contribute to the current data plane. Moreover, it can directly locates testing gaps to specific lines, which enables an efficient way of test development--creating new tests targeted to the testing gaps that can effectively improve coverage.

% A major challenge is that many network tests do not exercise configurations directly. Instead, they reason about the data plane state (e.g., forwarding tables or routing tables) produced by configurations. To answer which configuration elements are covered when a data plane element is tested, we need to consider what configuration elements contribute in producing it. Such mechanism is complicated for a handful of reasons. First, both direct and indirect contributions need to be tracked. In a distributed control plane, a piece of routing information may be propagated and transformed multiple times before arriving at its final location, and are thus jointly contributed by both local and non-local configurations. For example, the path attributes of a BGP route is shaped by routing policies on each and every hop that it traversed. Second, contribution comes in a variety of forms logically. Some forms of contribution are less significant than others. For example, when an aggregate route stems from multiple subnets, the contribution of each subnet is not necessary for the aggregate route to be present.

% Our solution is to model the contribution between configuration elements and data plane elements as an \textit{information flow graph}. An IFG is a directed acyclic graph (DAG) where vertices denote network elements and edges denote contributions. In addition to direct contributions from configuration elements to data plane elements, we also model contributions between data plane elements (from predecessors to successors). For instance, a BGP route contributes to the BGP message that derived from it. Indirect contributions are thus modeled by multi-hop paths in the DAG. We also combine graph structure with logic conjunction/disjunction to model the strong/weak contributions. 

% We build a tool called \sysname based on this model. \sysname computes configuration coverage using three inputs, the configurations, a stable data plane state, and the set of network elements\footnote{Both data plane elements and configuration elements are supported for completeness. The coverage computation for the latter is straightforward. An examples of network tests that directly analyze configurations is routing policy evaluation.} that are directly tested. The core of \sysname is a process to efficiently map any data plane element to the set of configuration elements that contribute to it. A key design choice of this process is to materialize the IFG lazily instead of tracking contributions proactively in producing the data plane. Such design has several advantages. First, it avoids the cost to compute and store contributions for transient or untested data plane elements. Second, \sysname is agnostic to the method of data plane generation and therefore supports a wider range of network testing/verification tools--data plane states used by different tools can be pulled from physical networks\cite{xx}, generated via simulation \cite{xx} or emulation \cite{xx}. Third, by computing coverage offline, \sysname does not require instrumentation of testing/verification tools and does not slow down test execution.

% \sysname supports configuration syntax for different vendors using a vendor-neutral model of configurations. It also supports a rich (but incomplete) set of configuration features such as interfaces, BGP peering and routing policies. Our implementation of \sysname reports configuration coverage in two easy-to-use formats, namely file-level statistics and line-level results as colored annotations on source configurations. \sysname is open source.

% %One potential approach to know information flow is to use do a high-fidelity simulation of the entire data plane and carefully trace the contributions in the process. It is non-ideal due to the high instrumentation and run-time overhead. Based on our observation that the static data plane state contains enough information to recover the information flow, we materialize the information flow model lazily. This also allows us to eliminate the cost for transient states and untested states.


% To demonstrate the value of using configuration coverage in network testing, we present a case study on Internet2, a nation-wide backbone network. By measuring configuration coverage of prior testing practices for this network, we found out that 63\% of configuration lines were actually untested. We also found out that coverage results produced by \sysname can locate meaningful testing gaps, so that test quality can be improved effectively and systematically.

% We benchmark the performance of \sysname on both realworld and synthetic networks. We find that \sysname scales reasonably. The time to compute coverage is 1.2 hours for the largest network that we used, which has 1 million forwarding rules. The time to compute coverage is less than 9\% compared to the time of test execution phase on all networks.



% %Analogous to code coverage in software testing, we analyzes which lines of router configurations are covered or nor covered during the execution of a test suite. The result can be used to quantify the rigorousness of the test suite and help discover the blind spots.



==> Control-Plane-Coverage [arxiv submission] (4)/sections/overview.tex <==
\section{Configuration Coverage: Overview}\label{sec:overview}


Network engineers today create data and control plane tests based on past outages and their knowledge of which behaviors are important to test. There are no tools to provide feedback on how well they are testing configurations and which aspects of the configuration are untested. We aim to build such a tool. Given the complexity of real-world networks, it is difficult for humans to know if they have covered all important elements of configurations.
%
As with software, high coverage is necessary but not sufficient for a good test suite.  In addition to exercising all key behaviors, the tests must also properly assert that those behaviors match intent. This latter task is not our focus.

We now outline how we compute which configuration elements are covered by a suite of data and control plane tests. 

\subsection{Defining coverage} 

We deem a configuration element to be covered if it $i)$ is tested directly by a control plane test; or $ii)$ contributes to the production of a data plane element tested by a data plane test. 
%The contributions in the production of a data plane element can be classified along three dimensions, namely local (on the same device as the data plane state) or non-local, deterministic or non-deterministic (when multiple contributors coexist), positive (to the acceptance of the data plane state) or negative (to the rejection of alternative data plane states). Our notion of configuration coverage considers both local and non-local, deterministic and non-deterministic (\cref{sec:weak_coverage}) contributions; on the third dimension, we consider only positive contributions and disregard negative ones. We make this design choice based on the meaningfulness of coverage results and computational cost.
For now, assume that contributions are deterministic. We discuss non-deterministic contributions in the next section.

\autoref{fig:coverage-example} illustrates configuration coverage as a result of a data plane test. It shows parts of the two routers' configuration. R1's configuration defines one interface (Lines 1-2) and one BGP peer (192.168.1.2, which is R2's address), and it specifies the import and export policy to use. The import policy (R2-to-R1 at Lines 6-11) denies routing messages for a particular prefix and sets the preference for another. 

R2's configuration defines two interfaces, a BGP peer (R1) and routing policies. At Line 13, it states that the prefix 10.10.1.0/24 should be announced to BGP peers {\em iff} it is in the main RIB.\footnote{Different router vendors have different semantics for BGP network statements. We are assuming Cisco semantics.} In our example, 10.10.1.0/24 will be in the main RIB as it corresponds to the eth1's prefix. (Address statements like Line 4 encode the IP address and prefix length. For eth1, given the address 10.10.1.1 and prefix length of 24, the prefix is 10.10.1.0/24.)
%
Routers add interface prefixes to the "connected" protocol RIB, from where those prefixes can enter the main RIB. The resulting RIBs on the two routers are shown in the figure. Each entry includes the next hop and source routing protocol ("conn" = connected). 

Suppose the entry for 10.10.1.0/24 at R1 was tested by a data plane test. The covered configuration elements are highlighted. On R1, the BGP peer configuration and import policy binding (Lines 3-4) are covered because the tested entry came via that peering and passed through that policy. Parts of the routing policy R2-to-R1 relevant to the tested state (Lines 6, 9-11) are also covered. The interface definition (Lines 1-2) is covered because it enables the BGP peering to be established. In contrast, the export policy R1-to-R2 and unexercised parts of R2-to-R1 (Lines 7-8) are not covered. 

There are covered configuration elements at R2 as well. These include the interface definitions---eth0 enables the BGP edge and 10.10.1.0/24 was announced due to eth1---and BGP peering, the export policy, and the BGP network statement.

\para{Alternative definitions of coverage}
One may consider an alternative definitions of coverage that disregards non-local configuration elements. But we posit that including non-local elements is more meaningful. These elements, such as the BGP network statement on R2's Line 13, are just as key to the existence of 10.10.1.0/24 at R1 as the local elements. 

Another definition of coverage is based on mutation~\cite{mutation-coverage}: a configuration line is covered if its mutation alters the test result. 
%In the networking context, example statements that this definition will deems as covered, which our chosen definition will not, include those that de-prioritize (or reject) alternative routes. Mutating the de-prioritization statements can change the test result. 
This definition will report an additional class of configuration elements as covered---configuration elements that de-prioritize (or reject) the competitors of the tested data plane element. 
Mutation-based coverage tends to be significantly harder to compute~\cite{mutation-survey}, and its results can be hard to interpret. In developing the first tool in this space, we decided to focus on a simpler, more direct definition of coverage. We will explore more sophisticated definitions in the future.

% de-prioritization  de-prioritization allows the   consider negative contributions that lead to the rejection of a better data plane states than the tested one. For example, suppose R2 announces 10.10.1.0/30 to R1, if there were not the import policy clause at R1's Lines 7-8, this route would be accepted by R1 and would override the route to 10.10.1.0/24 (according to longest prefix match). We choose not to offer a negative-contribution-aware metric because it is not tractably computable.

% Another definition of coverage may consider negative contributions that lead to the rejection of a better data plane states than the tested one. For example, suppose R2 announces 10.10.1.0/30 to R1, if there were not the import policy clause at R1's Lines 7-8, this route would be accepted by R1 and would override the route to 10.10.1.0/24 (according to longest prefix match). We choose not to offer a negative-contribution-aware metric because it is not tractably computable.

%\xieyang{expand this para into a dedicated discussion? May include negative contributions as well. There is a spectrum of ways to define contributions, and we need to balance meaningfulness and computational cost}



\begin{figure}[t!]
  \centering
    \includegraphics[width=\columnwidth]{figures/coverage-example.png}
    %\vspace{-20pt}
    \caption{An example network with routing tables and configurations. The highlighted configuration lines are covered when the route to 10.10.1.0/24 is tested at R1.}
    \label{fig:coverage-example}
\end{figure}

\subsection{Our approach}
%\para{Challenges in computing coverage}
While it is straightforward to identify configuration elements covered by a control plane test, it is not for data plane tests. 
%
Data plane tests analyze the "output" of the control plane, and we need a scalable way to compute which configuration elements contributed to tested data plane state. The relationship between these inputs and outputs is complex. How a particular RIB entry comes about relies on many configuration elements across multiple devices. 
%Inversely, a particular configuration element will impact numerous RIB entries. 
The need to map tested outputs to input space sets computation of configuration coverage apart from data plane coverage and software coverage, for both of which the coverage domain is the same as test domain.

% First, data plane is the output of control plane. Revealing the untested blind spots in the output does not reveal the blind spots in configurations themselves directly. There is a gap that we need to map from the output to the corresponding configuration lines. Moreover, the blind spot reported in terms of untested configuration blocks instead of generated data plane states are more interpretable by human operators.

% Second, the comprehensiveness of control plane verification should be considered and measured among all possible environments, while the data plane metrics assume a fixed environment. Even 100 \% data plane coverage under a fixed specific does not necessarily indicate the configuration being thoroughly tested. Some configuration blocks can only be tested under specific external announcements (such as the latent bug in the previous example) or failure conditions. 

To motivate our approach to solving this problem, let us first sketch two strawman approaches. 
One potential approach is to express control plane computation  declaratively, e.g., in Datalog. This enables identification of contributing inputs for a given output using a form of backward-reasoning~\cite{positiveprovenance,negativeprovenance}.
However, network control plane computations can be quite complex (e.g., non-monotonic behaviors \cite{stablepath, pathvector}). While declarative encodings may work in special cases~\cite{fastplane}, it is hard to get high-fidelty, performant encodings for the general case. 
%\xieyang{Indeed, we tried to put all dependency templates in a declarative framework, but failed due to the lack of expressiveness for some operations.} 
That is why most control plane analysis tools use an imperative approach~\cite{hoyan,batfish,plankton,cbgp}.\footnote{Batfish~\cite{batfish}, a widely used control plane analysis tool, originally used Datalog to encode network control planes but switched to imperative simulations due to expressiveness and performance challenges.}
%\xieyang{For fair comparison, I suppose we are comparing with \cite{negativeprovenance} in this paragraph, which introduces backward reasoning. Backward reasoning solves all three disadvantages of tracing-based approach but it is limited to declarative encoding. Our hybrid reasoning keeps these advantages, and plus it is general and independent of the control plane encoding.}

Another potential approach is to use simulation-based forward reasoning, i.e., simulate the control plane (imperatively) and track which configuration elements feed into each part of the data plane state. 
%In Figure~\ref{fig:coverage-example}, this means tagging the route to 10.10.1.0/24 at R1 with all the configuration elements that led to its production. 
However, this approach has scalability limitations.  Network simulation is time and memory intensive~\cite{batfish,hoyan,cbgp}, and it will become significantly worse if it needed to track all necessary information along each hop. 
%Applicability of this approach is also limited to networks for which a high-fidelity simulator is available.
%A simulation-based approach also 

%\xieyang{To make it a fair statement, we need to consider reference-based provenance~\cite{positiveprovenance}. They avoid the accumulation by only keeping the pointers to immediate parents. The full provenance can be retrieved lazily by doing a backward traversal along these pointers.} Any optimizations we might do, e.g., using Bloom filters to reduce memory needs~\cite{xx}, will make tracking imprecise and will likely over- or under-estimate coverage.
%\xieyang{We can argue three advantages against tracing-based approach. First, transient states don't have to be tracked (my question: is it significant for stable-path-focused verifiers such as Batfish?). Second, untested states don't have to be tracked. Third, our computation is offline and do not block critical path.}

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.9\linewidth]{figures/ifg_example.png}
    \caption{Subset of IFG for the \autoref{fig:coverage-example} example, to track configuration elements  on both routers that contribute to the tested RIB entry (F1). Colors denote different fact types: data plane state (white), configuration elements (yellow), auxiliary facts (green).}
    \label{fig:coverage-graph}
\end{figure*}

Our approach is based on two observations. First, for the purposes of computing coverage, we do not need a full computational model of the control plane. We need to only track which configuration elements contribute to tested data plane state (i.e., taint analysis~\cite{taj}), not the exact input-output relationship; and we need to reason only about the stable state (i.e., the the of devices once they have settled on best paths), not the transient states. Data plane testing~\cite{hsa,veriflow,deltanet,atomic,rcdc} assumes that the analyzed state is stable.
%\footnote{It is theoretically possible for a data plane test to  encounter transient state. Such occurrences are dealt via other methods, e.g., ignoring transient test failures~\cite{pingmesh}. Similar methods can be applied to coverage computation.}
%
Our second observation is that the stable state contains enough information for us to infer contributions of configuration elements after the fact, based on the semantics of the control plane. This inference is vastly cheaper than tracking contributions towards all data plane state entries, independent of whether they are tested.

%Our approach differs from these prior approaches in two ways. \xieyang{This claim sounds vague to me, as our approach solves different disadvantages of different prior approaches. We can start with the following argument here: we solved the disadvantages of both prior approaches and our approach is both general (regarding the underlying control plane encoding) and fast.} It uses a simpler model of network control planes \xieyang{it is also important that the model is independent of the model and encoding used by the verification tool}, and it uses hybrid backward-forward reasoning. 
%\xieyang{The hybrid reasoning is the key to solve the disadvantages of prior approaches. The stable-path model is a difference, but it is not an extra because its performance advantage on transient states is shared by backward reasoning. I think we can move the stable-path point to somewhere later.}

% Stable state information flow is simpler because it excludes transient states (non-best paths). Transient states are not relevant for coverage computation, allowing us to use a simpler model than prior approaches which capture the full computation.%\xieyang{The stable-path view is an important point that differentiate our method, but I think it may distract readers from appreciating how our methods combines the strength of both prior approaches. What about moving the stable-path point to somewhere later?}

To model and infer contributions to the stable state, we use an {\em information flow graph} (IFG). 
%
\autoref{fig:coverage-graph} shows a simplified subset of IFG for the \autoref{fig:coverage-example} example. Each node is a {\em fact} and each arrow denotes direct information flow from the tail to head. IFGs have three types of facts: $i)$ data plane state, $ii)$ configuration elements; and $iii)$ auxiliary facts that help connect the previous two types. 

The main RIB entry 10.10.1.0/24 at R1 (F1) is derived from the corresponding BGP RIB entry (F5),
%\footnote{In practice, devices also have a main RIB that stores best paths across routing protocols and information flows from there to the FIB. Our presentation omits this intermediate layer for simplicity.} 
which in turn is derived from the BGP message from R2 (F10). This message exists because of the BGP edge between R1 and R2 (F13), the source message sent by R2 (F11), and the relevant configuration element within import policy (F20). R2 sent the BGP message because of the same BGP edge (F13), its export policy elements (F22), and the BGP RIB entry (F7). This BGP RIB entry exists because of the configuration element (F23) and the RIB entry (F3), which exists because of the connected route (F8). The BGP edge (F13) exists because of the configuration elements that define the peering (F16, F17) and paths between R2 and R1 that enable the BGP session to be established. The paths depend on the RIB entries (F2 and F4, respectively), the contributions to which can be similarly traced. In this manner, the IFG captures all configuration elements that led to the tested RIB entry (F1).

%IFG dependencies are not tracked proactively, but we infer them on demand based on control plane semantics, using a mix of backward-forward reasoning. Backward inference infer the parent (tail) of the edge from its child (head). For instance, we can compute the RIB entry F6 from the FIB entry F2---the FIB entry indicates that the source routing protocol is BGP, and we thus look up the BGP RIB for 10.10.1.0/24.
We do not track IFG dependencies proactively but infer them on-demand based on control plane semantics, using a mix of backward-forward reasoning. 
%Backward inference is global--our goal is to infer the parent (tail) of the edge from its child (head) and recursively discover all ancestor nodes that lead to the child; Forward inference is local. 
Backward inference infers the parent (tail) of the edge from its child (head).
The information in child nodes is not enough to fully recover the parent nodes, but is often enough to select them from the known stable state. For instance, we can compute the BGP RIB entry F5 from the main RIB entry F1---the main RIB entry indicates that its source routing protocol is BGP, and we thus look up the BGP RIB for 10.10.1.0/24.

%Selecting the parents is not always straightforward; not all parents are available from the stable state. For instance, given a BGP message (F10) which has passed through an import policy, we can not directly know which policy terms of the import policy were exercised. Instead, we need to know--the pre-import BGP message (F11), the import policy of the BGP edge (F13) and trace the policy evaluation. Moreover, F11 is not part of the input and needs to be computed on-the-fly. To address these challenges, we complements backward inference in two ways.
%First, we allow backward inference to look ahead. For instance, given the post-import BGP message at R1 (F10), we can skip its immediate parent (F11) and look for its grandparent--the corresponding BGP route at R2 (F7). Second, we use targeted simulations to compute routing messages on-the-fly and to trace the policy terms exercised in this process.



%sometimes child nodes do not contain enough information to uniquely identify its parents within the stable state, so we compute them on-the-fly via targeted single-step simulations.

Lookup-based inference does not always work. For instance, given a BGP message which has passed through an import policy, we can not compute backwards which policy terms of the import policy were exercised (F10 $\leftarrow$ F20). Another parent of F10, the pre-import BGP message (F11) cannot be looked up either because it is not part of the input and needs to be computed on-the-fly. 
%We use two additional types of inferences to solve this challenge. The first one generalizes backward inference to indirect ancestors. For instance, given the post-import BGP message at R1 (F10), we can skip its immediate parent (F11) and look for its grandparent--the corresponding BGP route at R2 (F7). The second type of inference is forward inference. 
To address these limitations, we combine backward and forward inference. When a parent can not be directly looked up, we first look up the prerequisites of the parent. For instance, we can look up F7 based on F10. Next, we use targeted simulations to compute non-existing facts and to select relevant facts exercised in a control plane process or data plane process. For instance, given the BGP route at R2 (F7), we simulate its processing through the export policy, which allows us to derive the pre-import BGP message (F11) and find the policy term exercised during the export process (F22). Once F11 is computed, we conduct another targeted simulation to discover the policy term exercised in the import process (F20).
%
Unlike a full control plane simulation, these targeted simulations are fast. They have limited scope (e.g., best path selection is not simulated) and are done only for messages of interest, not all messages.

By combining backward and forward inference, atop the stable state IFG, we can scalably discover all covered configuration elements. We describe this approach in detail next.

% Backward reasoning is global. It utilizes information already present in the data plane state to link the tested data plane state element to all other data plane state elements that lead to it \xieyang{``all other routes that lead to it'' may confuse readers here. Conceptually a route is linked to its immediate parents, rather than other indirect ancestors.}. Forward reasoning is local to a device or an edge. Given a data plane state element, it uses targeted simulations to compute which configuration elements are invoked in its processing. \xieyang{This framing is great, the only thing is that the partition between forward and backward reasoning seems to be imprecise. It reads like backward is just for route <- route, forward is just for route <- config. To my understanding, some route <- route mappings are computed using local-forward-simulation, such as deriving an route announcement using its predecessor bgp route; some route <- config mappings are computed using backward reasoning, such as mapping from a bgp route to the network statement in config.}

%\xieyang{I suggest the following partition, that we use backward reasoning where we can, but fall back to forward, localized simulations when information are not available for us. In the scenarios when forward simulation is necessary, the nodes that await for simulation results can be ``skipped'' so that it won't block the global backward reasoning. For example, we link a bgp route directly to the route in neighbor's bgp rib (skipping the intermediate route announcement, which will be inserted between two bgp routes after the local-forward-simulation are done).}

%Consider the example in Figure~\ref{fig:coverage-example} again, in which route 10.10.0.0/24 at R2 was tested. Based on the available next hop information, we can link this route to the one at R1 and then to the one at R2. This linking is the key aspect of global backward reasoning. Given the route at R2, we can link it to the peer definition to R1 (line 1) and the import policy association (line 2, 4). Similarly, we can link to peer definitions and policy associations at R1 and R2. 

%To compute which lines of import and export policies were exercised, we run local simulations. At R2, we simulate the export policy R2-to-R1 on its route 10.10.0.0/24. This simulation yields that the line "permit 10.10.0.0/24" in the policy was exercised, and it also yields the exact routing message to R1 (in case the export policy changes a route attribute). Simulating this route on the import policy R2-to-R1 at R1 yields the line exercised in that policy. Finally, similar simulations across the R1-R2 edge, starting from the route at R1, yield exercised lines in the R1-to-R2 export policy at R1 and R1-to-R2 import policy at R2. Unlike the global simulations done from scratch~\cite{xx}, these local simulations are quite fast. They do not track non-local information, are limited in scope (e.g., best path selection is not simulated); and are done only for messages of interest, not all messages.

% In this work, we focus on a most basic form of control plane coverage, informally described as what lines of network configuration are covered by a test suite. \ryan{this definition seems circular} To answer this question, we first need to define what it means by ``covered'' in the context of network control plane verification. 

% And as we will show in this section, the definition of coverage is non-trivial due to two reasons. First, the tests used by control plane verification operate on the output of configurations, \EG, RIBs and FIBs, instead of executing them directly. Therefore \textit{the coverage of configuration is implied by coverage of routes}. Second, control plane routes have dependency and competition relations with each other, so that \textit{the coverage of a route may be implied by the coverage of other routes}.

% We propose a framework to define and compute control plane coverage, rather than defining a single metric. Our coverage framework is based on a general model of networks across control plane and data plane. Our model captures three mechanisms that are key to control plane coverage. First, what are the states of the network, and how do network tests operate on network states. Second, how do network states relate with each other, more specifically, if a network state is tested, does it implies some other states being (indirectly) tested. Third, how do network configurations contribute in the provenance of network states.

==> Control-Plane-Coverage [arxiv submission] (4)/sections/related.tex <==
\section{Related Work} 
\label{sec:related}

Our work builds on top of four lines of research.

\para{Code coverage}
We borrow from the software domain the idea of using code coverage to reveal testing gaps, quantify test suite quality, and help engineers improve their test suites~\cite{branch-coverage,mutation-coverage,overview-coverage}. Our coverage analysis techniques, however, are specialized to the operation of network configurations. 

\para{Data plane coverage}
Yardstick introduced data plane coverage metrics \cite{yardstick} that quantify the proportion of data plane elements such as forwarding rules and paths that are exercised by network tests. Configuration coverage goes further and maps tested data plane components to configuration elements that contribute to them. It provides more direct feedback because network engineers author configurations, not data plane state, and it supports testing of configuration elements that are not exercised by the current data plane state.  

\para{Network testing and verification}
A range of tools can analyse properties of network data and control planes~\cite{pingmesh,rcdc,hsa,batfish,hoyan,veriflow,deltanet,atomic,minesweeper,arc}.
%Data plane verification takes as input the network's data plane state (FIBs and ACLs) and determines if its reachability properties are as intended by operators. Data plane verification reasons about the output of configurations, hence it requires either collecting FIB snapshots after the deployment of configurations, or a simulator/emulator to generate the target data plane from configurations.
%Control plane verification makes stronger correctness guarantees by checking properties on both the current and ``future'' data planes caused by environment changes and thus verifies the logic encoded by the configurations more comprehensively. For example, they check reachability under arbitrary k failures.
\sysname borrows ideas from verification tools to concisely model the network, \EG, focusing on stable state and routing protocol instances~\cite{minesweeper,arc}. However, \sysname target a different problem---reveal what is tested vs enabling testing of new properties--and uses different techniques.

\para{Network provenance} 
Provenance systems can track causal dependencies of events in distributed systems.
Provenance systems like ExSPAN \cite{positiveprovenance} materialize provenance graphs by tracing system execution in forward direction.
%: while the distributed system is executing, they record the forward-direction derivation of system state tuples using some graph representation, and they respond to queries by projecting out the relevant subtree. The provenance relations are either stored as values (keep an entire subtree with each node) or references (keep pointers to immediate parent nodes). 
%Value-based provenance offers immediate provenance resolution at the cost of high storage overhead and high communication overhead in distributed systems. 
%Reference-based provenance fetches complete provenance of queried nodes on-demand by recursively resolving the provenance using pointers to immediate parent nodes until base facts.
Negative provenance systems can reason about missing events \cite{negativeprovenance} and materialize provenance graphs lazily using backward inference.
%, however, they rely on a declarative implementation of the network and a full log of control plane execution. 
\sysname too uses a graph-based model. However, it is unique in terms of accommodating network configuration into a provenance model, and this model, tailored to the stable state assumption, is more succinct. Further, it combines backward and forward inference to overcome the limitations of using only one type of inference. 

%making it not only efficient but also agnostic to control plane implementations. 

%The negative provenance graph is typically infinite and cannot be materialized. The derivation relations are inferred backwards using a set of construction algorithms. The algorithms are made by doing counterfactual reasoning on tuple derivation rules.
%We share the idea of backward graph construction with negative provenance work. However, our approach does not rely on a complete log of messages and events. The facts used by their model are just the transient states of the system, while we focus on the converged state and model more facts such as configurations and behaviors.
%This approach can be applied to both positive and negative provenance. However it does not work for control plane coverage. The reason is two-fold. First, we cannot have the complete derivation trace by instrumenting the system because most control plane verifiers do not simulate intermediate states with high fidelity. Second, their model is purely relational and only model system states, ie, routes, in our context, and thus cannot be used to model dependencies between routes and configs. 
